Distributed Binary Detection with Lossy Data Compression

Consider the problem where a statistician in a two-node system receives rate-limited information from a transmitter about marginal observations of a memoryless process generated from two possible distributions. Using its own observations, this receiver is required to first identify the legitimacy of its sender by declaring the joint distribution of the process, and then depending on such authentication it generates the adequate reconstruction of the observations satisfying an average per-letter distortion. The performance of this setup is investigated through the corresponding rate-error-distortion region describing the trade-off between: the communication rate, the error exponent induced by the detection and the distortion incurred by the source reconstruction. In the special case of testing against independence, where the alternative hypothesis implies that the sources are independent, the optimal rate-error-distortion region is characterized. An application example to binary symmetric sources is given subsequently and the explicit expression for the rate-error-distortion region is provided as well. The case of "general hypotheses" is also investigated. A new achievable rate-error-distortion region is derived based on the use of non-asymptotic binning, improving the quality of communicated descriptions. Further improvement of performance in the general case is shown to be possible when the requirement of source reconstruction is relaxed, which stands in contrast to the case of general hypotheses.

==> Final copy/commandes-2.tex <==


%--------------------------------------------------------------------
% ensembles
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\sE}{{\mathsf E}}

%\newcommand{\bP}{{\mathbb P}}
\newcommand{\bN}{{\mathbb N}}
\newcommand{\bC}{{\mathbb C}}
\newcommand{\bR}{{\mathbb R}}
\newcommand{\bZ}{{\mathbb Z}}

\newcommand{\sX}{{\mathsf X}}
\newcommand{\sY}{{\mathsf Y}}
\newcommand{\sS}{{\mathsf S}}
\newcommand{\snr}{{\textrm{snr}}}


%------------------------------------------------------------------------------
% intervalles FR [a;b], (a;b], [a;b) ou (a;b)
\newcommand{\intervalFR}[4]{\mathopen{#1}#2\mathclose{}\mathpunct{};#3\mathclose{#4}}
\newcommand{\intervalFRLR}[4]{\left #1 #2\mathpunct{};#3\right #4}

% intervalles ISO 31-11 [a,b], (a,b], [a,b) ou (a,b)
\newcommand{\interval}[4]{\mathopen{#1}#2\mathclose{},#3\mathclose{#4}}
\newcommand{\intervalLR}[4]{\left #1 #2,#3\right #4}

\newcommand{\intFF}[2]{\interval{[}{#1}{#2}{]}}
\newcommand{\intOF}[2]{\interval{(}{#1}{#2}{]}}
\newcommand{\intFO}[2]{\interval{[}{#1}{#2}{)}}
\newcommand{\intOO}[2]{\interval{(}{#1}{#2}{)}}

\newcommand{\intFFLR}[2]{\intervalLR{[}{#1}{#2}{]}}
\newcommand{\intOFLR}[2]{\intervalLR{(}{#1}{#2}{]}}
\newcommand{\intFOLR}[2]{\intervalLR{[}{#1}{#2}{)}}
\newcommand{\intOOLR}[2]{\intervalLR{(}{#1}{#2}{)}}


%------------------------------------------------------------------------------ 
% probabilité
\newcommand{\pr}[1]{\operatorname{Pr}\left\{#1\right\}}

% proba et espérance
\newcommand{\bE}{{\mathbb E}}
\newcommand{\bP}{{\mathbb P}}

% variance Var[.]
\newcommand{\Var}[1]{\text{Var}\left[#1\right]}

% variables aléatoires indépendantes
\newcommand{\indpt}{\perp\!\!\!\perp}

% chaîne de Markov
\newcommand{\mkv}{-\!\!\!\!\minuso\!\!\!\!-}

% relation d'ordre pour "less noisy"
\newcommand{\lessnoisy}[1]{\succeq_{\scriptscriptstyle #1}}

% ensemble typique
\newcommand{\typ}[2]{T_\delta^{#1}(#2)}

% barre au-dessus du texte pour exprimer l'événement complémentaire
\newcommand{\non}[1]{\stackrel{\_\_\_\_\_}{\text{#1}}}

% \sim pour variables i.i.d.
\newcommand{\simiid}{\stackrel{\text{i.i.d.}}{\sim}}

% loi uniforme sur un ensemble, loi de Bernoulli 
\newcommand{\unif}[1]{{\mathcal U}_{\,#1}}
\newcommand{\bern}{{\mathcal B}}

% loi normale
\newcommand{\cN}{{\mathcal N}}


%------------------------------------------------------------------------------
% transposée
\newcommand{\T}{^\text{\scshape{t}}}

%------------------------------------------------------------------------------
% norme et valeur absolue
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}


%------------------------------------------------------------------------------
% limite -> quand (.) tend vers (.)
\newcommand{\toas}[1]{\xrightarrow[#1]{}}


%------------------------------------------------------------------------------
% événement d'erreur
\newcommand{\err}{{\mathsf E}}
\newcommand{\Nerr}{\cancel{\mathsf E}}


%------------------------------------------------------------------------------
% indicatrice
\newcommand{\ind}[1]{\mathbf{1}_{#1}}


%------------------------------------------------------------------------------
% parties entières
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


==> Final copy/commandes.tex <==


%--------------------------------------------------------------------
% ensembles
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\sE}{{\mathsf E}}

%\newcommand{\bP}{{\mathbb P}}
\newcommand{\bN}{{\mathbb N}}
\newcommand{\bC}{{\mathbb C}}
\newcommand{\bR}{{\mathbb R}}
\newcommand{\bZ}{{\mathbb Z}}

\newcommand{\sX}{{\mathsf X}}
\newcommand{\sY}{{\mathsf Y}}
\newcommand{\sS}{{\mathsf S}}
\newcommand{\snr}{{\textrm{snr}}}


%------------------------------------------------------------------------------
% intervalles FR [a;b], (a;b], [a;b) ou (a;b)
\newcommand{\intervalFR}[4]{\mathopen{#1}#2\mathclose{}\mathpunct{};#3\mathclose{#4}}
\newcommand{\intervalFRLR}[4]{\left #1 #2\mathpunct{};#3\right #4}

% intervalles ISO 31-11 [a,b], (a,b], [a,b) ou (a,b)
\newcommand{\interval}[4]{\mathopen{#1}#2\mathclose{},#3\mathclose{#4}}
\newcommand{\intervalLR}[4]{\left #1 #2,#3\right #4}

\newcommand{\intFF}[2]{\interval{[}{#1}{#2}{]}}
\newcommand{\intOF}[2]{\interval{(}{#1}{#2}{]}}
\newcommand{\intFO}[2]{\interval{[}{#1}{#2}{)}}
\newcommand{\intOO}[2]{\interval{(}{#1}{#2}{)}}

\newcommand{\intFFLR}[2]{\intervalLR{[}{#1}{#2}{]}}
\newcommand{\intOFLR}[2]{\intervalLR{(}{#1}{#2}{]}}
\newcommand{\intFOLR}[2]{\intervalLR{[}{#1}{#2}{)}}
\newcommand{\intOOLR}[2]{\intervalLR{(}{#1}{#2}{)}}


%------------------------------------------------------------------------------ 
% probabilité
\newcommand{\pr}[1]{\operatorname{Pr}\left\{#1\right\}}

% proba et espérance
\newcommand{\bE}{{\mathbb E}}
\newcommand{\bP}{{\mathbb P}}

% variance Var[.]
\newcommand{\Var}[1]{\text{Var}\left[#1\right]}

% variables aléatoires indépendantes
\newcommand{\indpt}{\perp\!\!\!\perp}

% chaîne de Markov
\newcommand{\mkv}{-\!\!\!\!\minuso\!\!\!\!-}

% relation d'ordre pour "less noisy"
\newcommand{\lessnoisy}[1]{\succeq_{\scriptscriptstyle #1}}

% ensemble typique
\newcommand{\typ}[2]{T_\delta^{#1}(#2)}

% barre au-dessus du texte pour exprimer l'événement complémentaire
\newcommand{\non}[1]{\stackrel{\_\_\_\_\_}{\text{#1}}}

% \sim pour variables i.i.d.
\newcommand{\simiid}{\stackrel{\text{i.i.d.}}{\sim}}

% loi uniforme sur un ensemble, loi de Bernoulli 
\newcommand{\unif}[1]{{\mathcal U}_{\,#1}}
\newcommand{\bern}{{\mathcal B}}

% loi normale
\newcommand{\cN}{{\mathcal N}}


%------------------------------------------------------------------------------
% transposée
\newcommand{\T}{^\text{\scshape{t}}}

%------------------------------------------------------------------------------
% norme et valeur absolue
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}


%------------------------------------------------------------------------------
% limite -> quand (.) tend vers (.)
\newcommand{\toas}[1]{\xrightarrow[#1]{}}


%------------------------------------------------------------------------------
% événement d'erreur
\newcommand{\err}{{\mathsf E}}
\newcommand{\Nerr}{\cancel{\mathsf E}}


%------------------------------------------------------------------------------
% indicatrice
\newcommand{\ind}[1]{\mathbf{1}_{#1}}


%------------------------------------------------------------------------------
% parties entières
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


==> Final copy/defintions.tex <==

 \section{Strongly typical sequences and related results}
  \label{app:strongly}
  In this appendix we introduce standard notions in information theory but suited for the mathematical developments and proof needed in this work. The results presents can be easily derived from the standard formulations provided in~\cite{ELGamal-Kim-book} and~\cite{Csiszar81}. Be $\mathcal{X}$ and $\mathcal{Y} $  finite alphabets and $(x^n,y^n)\in\mathcal{X}^n\times \mathcal{Y}^n$.  With $\mathcal{P}(\mathcal{X}\times \mathcal{Y})$ we denote the set of all probability distributions on $\mathcal{X}\times\mathcal{Y}$. We define the \emph{strongly $\delta$-typical} sets as:
 
 \begin{definition}[Strongly typical set]
 Consider $p\in\mathcal{P}(\mathcal{X})$ and $\delta>0$. We say that $x^n\in\mathcal{X}^n$ is $p\delta$- strongly typical if $x^n\in\mathcal{T}_{[p]\delta}^n$ with:
 \begin{equation}
 \mathcal{T}_{[p]\delta}^n=\left\{x^n\in\mathcal{X}^n:\Big|\frac{N(a|x^n)}{n}-p(a)\Big|\leq\frac{\delta}{\|\mathcal{X}\|},\ \forall a\in\mathcal{X}\ \mbox{such that}\ p(a)\neq 0\right\}\ ,
 \label{eq:strong_delta_typ}
 \end{equation}
 where $N(a|x^n)$ denotes de number of occurrences of $a\in\mathcal{X}$ in $x^n$ and $p\in\mathcal{P}(\mathcal{X})$.  When $X\sim p_X(x)$ we can denote the corresponding set of strongly typical sequences as $\mathcal{T}_{[X]\delta}^n$. 
  \end{definition}
 Similarly, given $p_{XY}\in\mathcal{P}\left(\mathcal{X}\times\mathcal{Y}\right)$ we can construct the set of $\delta$-jointly typical sequences as:
  \begin{gather}
  \mathcal{T}_{[XY]\delta}^n=\left\{(x^n,y^n)\in\mathcal{X}^n\times\mathcal{Y}^n:\Big|\frac{N(a,b|x^n,y^n)}{n}-p_{XY}(a,b)\Big|\leq\frac{\delta}{\|\mathcal{X}\|\|\mathcal{Y}\|},\right.\nonumber\\
  \left.\ \forall (a,b)\in\mathcal{X}\times\mathcal{Y}\ \mbox{such that}\ p_{XY}(a,b)\neq 0\right\}\ .
  \label{eq:joint_strong_delta_typ}
  \end{gather}
 We also define the \emph{conditional} typical sequences. In precise terms, given $x^n\in\mathcal{X}^n$ we consider the set:
 \begin{gather}
 \mathcal{T}_{[Y|X]\delta}^n(x^n)=\Big\{y^n\in\mathcal{Y}^n:\Big|\frac{N(a,b|x^n,y^n)}{n}-p_{XY}(a,b)\Big|\leq\frac{\delta}{\|\mathcal{X}\|\|\mathcal{Y}\|},\nonumber\\
\ \forall (a,b)\in\mathcal{X}\times\mathcal{Y}\ \mbox{such that}\ p_{XY}(a,b)\neq 0\Big\}\ .
\label{eq:cond_strong_delta_typ}
 \end{gather} 
 Notice that we the following is an alternative writing of this set:
 \begin{equation} 
 \mathcal{T}_{[Y|X]\delta}^n(x^n)=\left\{y^n\in\mathcal{Y}^n:(x^n,y^n)\in\mathcal{T}_{[XY]\delta}^n\right\} \ .
 \end{equation}
 
 We have several useful and standard lemmas, which will be presented without proof (except for the last one):
 
 \begin{lemma}[Properties of typical sets~\cite{Csiszar81}] 
 The following are true:
 \begin{enumerate}
 \item  Consider $(x^n,y^n)\in\mathcal{T}_{[XY]\epsilon}^n$. Then, $x^n\in\mathcal{T}_{[X]\epsilon}^n$, $y^n\in\mathcal{T}_{[Y]\epsilon}$, $x^n\in\mathcal{T}_{[X|Y]\epsilon}^n(y^n)$ and $y^n\in\mathcal{T}_{[Y|X]\epsilon}^n(x^n)$ \ .
 \item Be $T_{[Y|X]\epsilon}^n(x^n)$ with $x^n\notin\mathcal{T}^n_{[X]\epsilon}$. Then $T_{[Y|X]\epsilon}^n(x^n)=\varnothing$ \ .
 \item Be $(X^n,Y^n)\sim\prod_{t=1}^np_{XY}(x_t,y_t)$. If $x^n\in\mathcal{T}_{[X]\epsilon}^n$ we have
 \[2^{-n(H(X)+\delta(\epsilon))}\leq p_{X^n}(x^n)\leq 2^{-n(H(X)-\delta(\epsilon))} \]
 with $\delta(\epsilon)\rightarrow 0$ when $\epsilon\rightarrow 0$. Similarly, if $y^n\in\mathcal{T}_{[Y|X]\epsilon}^n(x^n)$:
  \[2^{-n(H(Y|X)+\delta'(\epsilon))}\leq p_{Y^n|X^n}(y^n|x^n)\leq 2^{-n(H(Y|X)-\delta'(\epsilon))} \]
  with $\delta'(\epsilon)\rightarrow 0$ when $\epsilon\rightarrow 0$\ .
 \label{lemma:cont}
 \end{enumerate}
 \label{lemma:useful}
 \end{lemma}
 
 \begin{lemma}[Conditional typicality lemma~\cite{Csiszar81}]
 Consider de product measure $\prod_{t=1}^np_{XY}(x_t,y_t)$. Using that measure, we have the following 
 \[\operatorname{Pr}\left\{\mathcal{T}_{[X]\epsilon}^n\right\}\geq 1-\mathcal{O}\left(c_1^{-nf(\epsilon)}\right),\ \ c_1>1\]
 where $f(\epsilon)\rightarrow 0$ when $\epsilon\rightarrow 0$. In addition, for every  $x^n\in\mathcal{T}^n_{[X]\epsilon'}$ with $\epsilon'<\frac{\epsilon}{\|\mathcal{Y}\|}$ we have:
 \[\operatorname{Pr}\left\{\mathcal{T}_{[Y|X]\epsilon}^n(x^n)|x^n\right\}\geq 1-\mathcal{O}\left(c_2^{-ng(\epsilon,\epsilon')}\right),\ \ c_2>1\]
 where $g(\epsilon,\epsilon')\rightarrow 0$ when $\epsilon,\epsilon'\rightarrow 0$.
 \label{lemma:prob_lim}
 \end{lemma}
 
 \begin{lemma}[Size of typical sets~\cite{Csiszar81}]
Given $p_{XY}\in\mathcal{P}\left(\mathcal{X}\times\mathcal{Y}\right)$ we have
  \[\frac{1}{n}\|\mathcal{T}_{[X]\epsilon}^n\|\leq H(X)+\delta(\epsilon),\ \  \frac{1}{n}\|\mathcal{T}_{[X]\epsilon}^n\|\geq H(X)-\delta'(\epsilon,n)\]
  where $\delta(\epsilon),\delta'(\epsilon,n)\rightarrow 0$ when $\epsilon\rightarrow 0$ and $n\rightarrow\infty$. Similarly for every $x^n\in\mathcal{X}^n$ we have:
  \[\frac{1}{n}\|\mathcal{T}_{[Y|X]\epsilon}^n(x^n)\|\leq H(Y|X)+\delta(\epsilon)\]
  with $\delta(\epsilon)\rightarrow 0$ with $\epsilon\rightarrow 0$. In addition, for every $x^n\in\mathcal{T}_{[X]\epsilon'}^n$ with $\epsilon'<\frac{\epsilon}{\|\mathcal{Y}\|}$ we have:
    \[\frac{1}{n}\|\mathcal{T}_{[Y|X]\epsilon}^n(x^n)\|\geq H(Y|X)-\delta'(\epsilon,\epsilon',n)\]
 where $\delta'(\epsilon,\epsilon',n)\rightarrow 0$ when $\epsilon,\epsilon'\rightarrow 0$ and $n\rightarrow\infty$.
 \label{lemma:size}
 \end{lemma}
 
 \begin{lemma}[Joint typicality lemma~\cite{Csiszar81}]
 \label{lemma:joint_typ_strong}
 Consider $(X,Y,Z)\sim p_{XYZ}(x,y,z)$ and $(x^n,y^n)\in\mathcal{T}_{[XY]\epsilon'}^n$ with $\epsilon'<\frac{\epsilon}{\|\mathcal{Z}\|}$ and $\epsilon<\epsilon''$. If $p_{Z^n|X^n}(z^n|x^n)=\frac{\mathds{1}\left\{z^n\in\mathcal{T}_{[Z|X]\epsilon''}^n(x^n)\right\}}{\|\mathcal{T}_{[Z|X]\epsilon''}(x^n)\|}$ there exists $\delta'(\epsilon,\epsilon',\epsilon'',n)$ which goes to zero  as $\epsilon,\epsilon',\epsilon''\rightarrow 0$ and $n\rightarrow\infty$ and: 
 \[2^{-n(I(Y;Z|X)+\delta')}\leq\operatorname{Pr}\left\{\tilde{Z}^n\in\mathcal{T}_{[Z|XY]\epsilon}^n(x^n,y^n)\right\}\leq 2^{-n(I(Y;Z|X)-\delta')}\]
 \end{lemma}

\begin{lemma}[Covering Lemma~\cite{ELGamal-Kim-book}]
\label{lemma:covering}
Be $(U,V,X)\sim p_{UVX}$ and $(x^n,u^n)\in\mathcal{T}_{[XU]\epsilon'}^n$, $\epsilon'<\frac{\epsilon}{\|\mathcal{V}\|}$ and $\epsilon<\epsilon''$. Consider also $\left\{V^n(m)\right\}_{m=1}^{2^{nR}}$ random vectors  which are independently generated according to $\frac{\mathds{1}\left\{v^n\in\mathcal{T}_{[V|U]\epsilon''}^n(u^n)\right\}}{\|\mathcal{T}_{[V|U]\epsilon''}(u^n)\|}$. Then:
\begin{equation}
\mbox{Pr}\left\{V^n(m)\notin\mathcal{T}_{[V|UX]\epsilon}^n(x^n,u^n)\ \mbox{for all}\ m\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
uniformly for every  $(x^n,u^n)\in\mathcal{T}^n_{[XU]\epsilon'}$  if: 
\begin{equation}
R>I\left(V;X|U\right)+\delta(\epsilon,\epsilon',\epsilon'',n)
\label{eq:covering_lemma}
\end{equation}
where $\delta(\epsilon,\epsilon',\epsilon'',n)\rightarrow 0$ when $\epsilon,\epsilon',\epsilon''\rightarrow 0$ and $n\rightarrow \infty$.
\end{lemma}
\begin{corollary}
\label{coro:covering}
Assume the conditions in Lemma~\ref{lemma:covering}, and  also:
\begin{equation}
\mbox{Pr}\left\{\left(X^n,U^n\right)\in\mathcal{T}^n_{[XU]\epsilon'}\right\}\xrightarrow[n\rightarrow\infty]{}1\ .
\end{equation}
Then:
\begin{equation}
\mbox{Pr}\left\{\left(U^n,X^n,V^n(m))\right)\notin\mathcal{T}_{[UXV]\epsilon}^n\ \mbox{for all}\ m\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
when (\ref{eq:covering_lemma}) is satisfied.
\end{corollary}

\begin{lemma}[Packing Lemma~\cite{ELGamal-Kim-book}]
\label{lemma:packing}
Be $(U_1U_2WV_1V_2X)\sim p_{U_1U_2WV_1V_2X}$, $(x^n,w^n,v_1^n,v_2^n)\in\mathcal{T}^n_{[XWV_1V_2]\epsilon'}$ and  $\epsilon'<\frac{\epsilon}{\|\mathcal{U}_1\|\|\mathcal{U}_2\|}$ and $\epsilon<\min{\left\{\epsilon_1,\epsilon_2\right\}}$. Consider random vectors $\left\{U_1^n(m_1)\right\}_{m_1=1}^{\mathcal{A}_1}$ and $\left\{U_2^n(m_2)\right\}_{m_2=1}^{\mathcal{A}_2}$ which are independently generated according to 
\begin{equation*}
\frac{\mathds{1}\left\{u_i^n\in\mathcal{T}_{[U_i|V_iW]\epsilon_i}^n(v_i^n,w^n)\right\}}{\|\mathcal{T}_{[U_i|V_iW]\epsilon_i}(w^n,v_i^n)\|},\ i=1,2\ ,
\end{equation*}
and $\mathcal{A}_1,\mathcal{A}_2$ are positive random variables independent of everything else. Then
\begin{equation}
\mbox{Pr}\left\{\left(U_1^n(m_1),U_2^n(m_2)\right)\in\mathcal{T}_{[U_1U_1|XWV_1V_2]\epsilon}^n(x^n,w^n,v_1^n,v_2^n)\ \mbox{for some}\ (m_1,m_2)\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
uniformly for every  $(x^n,w^n,v_1^n,v_2^n)\in\mathcal{T}^n_{[XWV_1V_2]\epsilon'}$  provided that: 

\begin{equation}
\frac{\log{\mathbb{E}\left[\mathcal{A}_1\mathcal{A}_2\right]}}{n}<I\left(U_1;XV_2U_2|WV_1\right)+I\left(U_2;XV_1U_1|WV_2\right)-I\left(U_1;U_2|XWV_1V_2\right)-\delta
\label{eq:packing_lemma}
\end{equation}
where $\delta\equiv\delta(\epsilon,\epsilon',\epsilon_1,\epsilon_2,n)\rightarrow 0$ when $\epsilon,\epsilon',\epsilon_1,\epsilon_2\rightarrow 0$ and $n\rightarrow \infty$.
\end{lemma}

\begin{corollary}
\label{coro:packing}
Assume the conditions in Lemma~\ref{lemma:packing}, and  also:
\begin{equation}
\mbox{Pr}\left\{\left(X^n,W^n,V_1^n,V_2^n\right)\in\mathcal{T}^n_{[XWV_1V_2]\epsilon'}\right\}\xrightarrow[n\rightarrow\infty]{}1
\end{equation}
Then:
\begin{equation}
\mbox{Pr}\left\{\left(U_1^n(m_1),U_2^n(m_2),X^n,W^n,V_1^n,V_2^n)\right)\in\mathcal{T}_{[U_1U_1XWV_1V_2]\epsilon}^n\ \mbox{for some}\ (m_1,m_2)\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
when (\ref{eq:packing_lemma}) is satisfied.
\end{corollary}

\begin{lemma}[Generalized Markov Lemma~\cite{GML_ours_2014} ]
Consider a pmf $p_{UXY}$ belonging to $\mathcal{P}\left(\mathcal{X}\times\mathcal{Y}\times\mathcal{U}\right)$ and that satisfies de following:
\[Y\mkv X\mkv U\]
Consider $(x^n,y^n)\in\mathcal{T}^n_{[XY]\epsilon'}$ and random vectors $U^n$  generated according to:

\begin{equation}
\label{eq:u_dist}
\mbox{Pr}\left\{U^n=u^n\Big|x^n,y^n,U^n\in\mathcal{T}^n_{[U|X]\epsilon''}(x^n)\right\}=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|X]\epsilon''}^n(x^n)\right\}}{\|\mathcal{T}_{[U|X]\epsilon''}^n(x^n)\|}
\end{equation}
For sufficiently small $\epsilon,\epsilon',\epsilon''$ the following holds uniformly for every  $(x^n,y^n)\in\mathcal{T}^n_{[XY]\epsilon'}$:

\begin{equation}
\mbox{Pr}\left\{U^n\notin\mathcal{T}^n_{[U|XY]\epsilon}(x^n,y^n)\Big|x^n,y^n,U^n\in\mathcal{T}^n_{[U|X]\epsilon''}(x^n)\right\}=\mathcal{O}\left(c^{-n}\right)
\end{equation}
where $c>1$.
  \label{lemma:markov}
  \end{lemma}

%  \begin{lemma}[Markov Lemma]
%Consider a pmf $p_{UVXYZ}$ on a finite product alphabet $\mathcal{X}\times\mathcal{Y}\times\mathcal{Z}\times\mathcal{U}\times\mathcal{V}$ and that satifies de following:
%\[(UXZ)\mkv Y\mkv V,\ \ (VYZ)\mkv X\mkv U\]
%Consider $(x^n,y^n,z^n)\in\mathcal{T}^n_{[XYZ]\delta}$ and random vectors $U^n$ and $V^n$ generated according to:
%\[p_{U^nV^n|X^nY^nZ^n}(u^n,v^n|x^n,y^n,z^n)=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|X]\delta}^n(x^n)\right\}}{\|\mathcal{T}_{[U|X]\delta}^n(x^n)\|}\frac{\mathds{1}\left\{v^n\in\mathcal{T}_{[V|Y]\delta}^n(y^n)\right\}}{\|\mathcal{T}_{[V|Y]\delta}^n(y^n)\|}\]
%For sufficiently small $\delta$ and $\epsilon$ the following holds:
%\[\mbox{Pr}\left\{(U^n,V^n)\notin\mathcal{T}^n_{[UV|XYZ]\epsilon}(x^n,y^n,z^n)|x^n,y^n,z^n\right\}=\mathcal{O}\left(c^{-n}\right)\]
%where $c>1$.
%  \label{lemma:markov}
%  \end{lemma}
\begin{corollary}
\label{coro:markov}
Assume the conditions in Lemma~\ref{lemma:markov}, and also:
\begin{equation}
\mbox{Pr}\left\{\left(X^n,Y^n\right)\in\mathcal{T}^n_{[XY]\epsilon'}\right\}\xrightarrow[n\rightarrow\infty]{}1
\end{equation}
and that uniformly for every $(x^n,y^n)\in\mathcal{T}^n_{[XY]\epsilon'}$:
\begin{equation}
\mbox{Pr}\left\{U^n\notin\mathcal{T}^n_{[U|X]\epsilon''}(x^n)\Big| x^n,y^n\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
we obtain:
\begin{equation}
\mbox{Pr}\left\{(U^n,X^n,Y^n)\in\mathcal{T}^n_{[UXY]\epsilon}\right\}\xrightarrow[n\rightarrow\infty]{}1\ .
\end{equation}
\end{corollary}
 Lemma~\ref{lemma:markov} and Corollary~\ref{coro:markov} will be central for us. They will guarantee the joint typicality of the descriptions generated in different encoders considering the pmf of the chosen descriptions induced by the coding scheme used. 
 %See the differences with lemma \ref{lemma:prob_lim}. In fact, Markov lemma is more useful that \ref{lemma:prob_lim}, where the random vectors $U^n$ are generated through the product measure $\prod_{i=1}^np_{U|XY}(u_i|x_iy_i)=\prod_{i=1}^np_{U|X}(u_i|x_i)$. ç
 The original proof of this result is given in~\cite{PhD-Tung} and involves a combination of rather sophisticated algebraic and combinatorial arguments over finite alphabets. Alternative  proof was also provided  in~\cite{ELGamal-Kim-book}, 
 \begin{equation}
 \mbox{Pr}\left\{(U^nX^n,Y^n)\in\mathcal{T}^n_{[UXY]\epsilon}\right\}\xrightarrow[n\rightarrow\infty]{}1
 \end{equation}
which strongly relies on a rather obscure result by Uhlmann~\cite{Uhlmann} on combinatorics. In~\cite{GML_ours_2014} a short and more general proof of this result is given.

We next present a result which will be useful for proving theorem  \ref{theo-main-theorem}. In order to use the Markov lemma we need to show that the descriptions induced by the encoding procedure in each node satisfies (\ref{eq:u_dist}).
   \begin{lemma}[Encoding induced distribution]   \label{lemma:induced}
 Consider a pmf $p_{UXW}$ belonging to $\mathcal{P}\left(\mathcal{U}\times\mathcal{X}\times\mathcal{W}\right)$ and $\epsilon'\geq\epsilon$.  Be $\left\{U^n(m)\right\}_{m=1}^{S}$ random vectors independently generated according to 
 $$
 \frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|W]\epsilon'}^n(w^n)\right\}}{\|\mathcal{T}_{[U|W]\epsilon'}(w^n)\|}
 $$ 
 and where $(W^n,X^n)$ are generated with an arbitrary distribution. Once these vectors are generated, and given $x^n$ and $w^n$, we choose one of them if:
  \begin{equation}
  \left(u^n(m),w^n,x^n\right)\in\mathcal{T}^n_{[UWX]\epsilon},\ \mbox{for some}\ m\in[1:S] \ .\end{equation}
 If there are various vectors $u^n$ that satisfies this we choose the one with smallest index. If there are none we choose an arbitrary one. Let $M$ denote the index chosen. 
 %Assume that:
% \[\mbox{Pr}\left\{\left(U^n(m),W^n,X^n\right)\notin\mathcal{T}^n_{[UWX]\epsilon}\ \forall m\in[1:S]\right\}\xrightarrow[n\rightarrow\infty]{}0.\]
 Then we have that:
  \begin{equation}
 \mbox{Pr}\left\{U^n(M)=u^n\Big|x^n,w^n,U^n(M)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}=
 \frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|XW]\epsilon}^n(x^n,w^n)\right\}}{\|\mathcal{T}_{[U|XW]\epsilon}(x^n,w^n)\|} \ .
 \end{equation}
   \end{lemma}
   \begin{IEEEproof}
   From the selection procedure for $M$ we know that:
  \begin{equation}
  M=f\left(\mathds{1}\left\{(U^n(m),X^n,W^n)\in\mathcal{T}_{[UXW]\epsilon}^n\right\}, m\in[1:S]\right)\ , \end{equation}
   where $f(\cdot)$ is an appropriate function. Moreover, because of this and the way in which the random vectors $U^n$ are generated we have:
\begin{equation}
U^n(M)\mkv\left(\mathds{1}\left\{(U^n(M),X^n,W^n)\in\mathcal{T}_{[UXW]\epsilon}^n\right\},W^n,X^n\right)\mkv M\ .
\label{eq:mkv}
\end{equation}
We can write:
\begin{IEEEeqnarray}{lCl}
\mbox{Pr}\left\{U^n(M)=u^n\Big|x^n,w^n,U^n(M)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}=\nonumber\\
\sum_{m=1}^S\mbox{Pr}\left\{M=m\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}\times\nonumber\\
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n),M=m\right\}.
\label{eq:mkv2}
\end{IEEEeqnarray}
From (\ref{eq:mkv}), the second probability term in the RHS of (\ref{eq:mkv2}) can be written as:
\begin{equation}
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}\ \forall m\ .
\end{equation}
We are going to analyze this term. It is clear that we can write:
\begin{IEEEeqnarray}{rcl}
\mbox{Pr}\left\{U^n(m)=u^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\Big| x^n,w^n\right\} &=&
\mathds{1}\left\{u^n\in\mathcal{T}_{[U|WX]\epsilon}^n(x^n,w^n)\right\}\nonumber\\
& &\times\mbox{Pr}\left\{U^n(m)=u^n\Big| x^n,w^n\right\}\ \forall m\ .\,\,\, \,\, \, \,\, 
\end{IEEEeqnarray}
\end{IEEEproof}
This means that
\begin{gather}
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}\nonumber\\
=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|WX]\epsilon}^n(x^n,w^n)\cap\mathcal{T}_{[U|W]\epsilon'}^n(w^n)\right\}}{
\mbox{Pr}\left\{U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\Big| x^n,w^n\right\}\|\mathcal{T}_{[U|W]\epsilon'}(w^n)\|}\ \forall m
\label{eq:uniform_1}
\end{gather}
From (\ref{eq:uniform_1}) and the fact that for $\epsilon'\geq\epsilon$, we have that $\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\subseteq
\mathcal{T}^n_{[U|W]\epsilon'}(w^n)$ we obtain:
\begin{equation}
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}
=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|WX]\epsilon}^n(x^n,w^n)\right\}}
{\|\mathcal{T}_{[U|XW]\epsilon}(x^n,w^n)\|}\ \forall m\ .
\label{eq:uniform_2}
\end{equation}
From this equation and (\ref{eq:mkv2}) we easily obtain the desired result.

%------------------------------------------------------------------------------
%\subsection{Csisz\'ar and K\"orner's Equality}
%
%
%\begin{lemma}[{Csisz\'ar and K\"orner's equality~\cite[Lemma~7]\cite{csiszar1978broadcast}}]\label{sec:csiszarkorner}
%Consider two  sequences $X^n$ and $Y^n$, and a random variable $Z$ arbitrarly distributed.
%The following identity holds true:
%\[
%\sum_{i=1}^n I(Y_{i+1}^n ; X_i | Z X^{i-1})
%	=	\sum_{j=1}^n I(X^{j-1} ; Y_j | Z Y_{j+1}^n)	\ .
%\]
%\end{lemma}

We present, without proof, a useful result about reconstruction functions for lossy source coding problems:
\begin{lemma}[Reconstruction functions for degraded random variables \cite{kaspi_two-way_1985}]
\label{lemma:Markov_distortion}
Consider random variables $(X,Y,Z)$ such that $X\mkv Y\mkv Z$. Consider an arbitrary function $\hat{X}=f(Y,Z)$ and an arbitrary positive distortion function $d(\cdot,\cdot)$. Then $\exists\ g^{*}(Y)$ such that
\begin{equation}
E\left[d(X,g^{*}(Y))\right]\leq E[d(X,f(Y,Z))]\ .
\label{eq:best_dist_function}
\end{equation}
\end{lemma}


==> Final copy/figures/BSCGeneral.tex <==


\begin{tikzpicture}
	\begin{axis}[
	title = \textbf{},
		xlabel=$\delta$,
		ylabel=,
		xmin = 0,
		ymin = 0,
		xmax = 0.18,
		ymax = 0.2]
		\pgfplotsset{every axis legend/.append style={
at={(0.02,0.98),font = \small},
anchor= north west}}



%	\addplot[blue,line width=1pt] coordinates {
%(0.500,0.681) (0.600,0.615) (0.700,0.566) (0.800,0.529) (0.900,0.499) (1.000,0.475) (1.100,0.455) (1.200,0.438) (1.300,0.424) (1.400,0.411) (1.500,0.401) (1.600,0.391) (1.700,0.383) (1.800,0.375) (1.900,0.368) (2.000,0.362) (2.100,0.357) (2.200,0.352) (2.300,0.347) (2.400,0.343) 
%	};
%	
%	\addplot[red,line width=1pt] coordinates {
%(0.500,0.613) (0.600,0.543) (0.700,0.491) (0.800,0.452) (0.900,0.421) (1.000,0.396) (1.100,0.375) (1.200,0.358) (1.300,0.343) (1.400,0.330) (1.500,0.319) (1.600,0.310) (1.700,0.301) (1.800,0.294) (1.900,0.287) (2.000,0.281) (2.100,0.275) (2.200,0.270) (2.300,0.266) (2.400,0.261) 
%	};
	
%	\addplot[black,dotted,line width=1pt] coordinates {
%(1.100,0.346) (1.200,0.329) (1.300,0.314) (1.400,0.301) (1.500,0.289) (1.600,0.278) (1.700,0.268) (1.800,0.260) (1.900,0.252) (2.000,0.244) (2.100,0.238) (2.200,0.231) (2.300,0.226) (2.400,0.220) (2.500,0.215) (2.600,0.211) (2.700,0.206) (2.800,0.202) (2.900,0.199) (3.000,0.195) 
%	};

%\draw[fill=gray!50,opacity=.7]
%(axis cs:0,0) -- (axis cs:0.0815,0) -- (axis cs:0.0815,0.2) -- (axis cs:0,0.2) -- cycle ;

\addplot[black,line width = 1pt] coordinates{
( 0.00100503, 0.05253741)( 0.00201005, 0.05214594)( 0.00301508, 0.05175804)( 0.00402010, 0.05137366)( 0.00502513, 0.05099275)( 0.00603015, 0.05061526)( 0.00703518, 0.05024115)( 0.00804020, 0.04987038)( 0.00904523, 0.04950289)( 0.01005025, 0.04913865)( 0.01105528, 0.04877762)( 0.01206030, 0.04841974)( 0.01306533, 0.04806499)( 0.01407035, 0.04771332)( 0.01507538, 0.04736469)( 0.01608040, 0.04701906)( 0.01708543, 0.04667639)( 0.01809045, 0.04633665)( 0.01909548, 0.04599980)( 0.02010050, 0.04566580)( 0.02110553, 0.04533463)( 0.02211055, 0.04500623)( 0.02311558, 0.04468059)( 0.02412060, 0.04435766)( 0.02512563, 0.04403741)( 0.02613065, 0.04371981)( 0.02713568, 0.04340483)( 0.02814070, 0.04309244)( 0.02914573, 0.04278260)( 0.03015075, 0.04247529)( 0.03115578, 0.04217048)( 0.03216080, 0.04186813)( 0.03316583, 0.04156821)( 0.03417085, 0.04127071)( 0.03517588, 0.04097559)( 0.03618090, 0.04068282)( 0.03718593, 0.04039238)( 0.03819095, 0.04010424)( 0.03919598, 0.03981837)( 0.04020101, 0.03953475)( 0.04120603, 0.03925336)( 0.04221106, 0.03897416)( 0.04321608, 0.03869713)( 0.04422111, 0.03842226)( 0.04522613, 0.03814951)( 0.04623116, 0.03787887)( 0.04723618, 0.03761030)( 0.04824121, 0.03734379)( 0.04924623, 0.03707931)( 0.05025126, 0.03681685)( 0.05125628, 0.03655638)( 0.05226131, 0.03629788)( 0.05326633, 0.03604132)( 0.05427136, 0.03578670)( 0.05527638, 0.03553398)( 0.05628141, 0.03528315)( 0.05728643, 0.03503418)( 0.05829146, 0.03478707)( 0.05929648, 0.03454178)( 0.06030151, 0.03429831)( 0.06130653, 0.03405662)( 0.06231156, 0.03381671)( 0.06331658, 0.03357856)( 0.06432161, 0.03334214)( 0.06532663, 0.03310744)( 0.06633166, 0.03287445)( 0.06733668, 0.03264314)( 0.06834171, 0.03241349)( 0.06934673, 0.03218550)( 0.07035176, 0.03195915)( 0.07135678, 0.03173441)( 0.07236181, 0.03151128)( 0.07336683, 0.03128974)( 0.07437186, 0.03106977)( 0.07537688, 0.03085136)( 0.07638191, 0.03063448)( 0.07738693, 0.03041914)( 0.07839196, 0.03020531)( 0.07939698, 0.02999298)( 0.08040201, 0.02978213)( 0.08140704, 0.02957275)( 0.08241206, 0.02936482)( 0.08341709, 0.02915834)( 0.08442211, 0.02895329)( 0.08542714, 0.02874965)( 0.08643216, 0.02854742)( 0.08743719, 0.02834658)( 0.08844221, 0.02814711)( 0.08944724, 0.02794901)( 0.09045226, 0.02775225)( 0.09145729, 0.02755684)( 0.09246231, 0.02736276)( 0.09346734, 0.02716999)( 0.09447236, 0.02697852)( 0.09547739, 0.02678834)( 0.09648241, 0.02659945)( 0.09748744, 0.02641182)( 0.09849246, 0.02622545)( 0.09949749, 0.02604033)( 0.10050251, 0.02585645)( 0.10150754, 0.02567378)( 0.10251256, 0.02549234)( 0.10351759, 0.02531209)( 0.10452261, 0.02513304)( 0.10552764, 0.02495517)( 0.10653266, 0.02477847)( 0.10753769, 0.02460294)( 0.10854271, 0.02442856)( 0.10954774, 0.02425532)( 0.11055276, 0.02408322)( 0.11155779, 0.02391223)( 0.11256281, 0.02374237)( 0.11356784, 0.02357360)( 0.11457286, 0.02340594)( 0.11557789, 0.02323936)( 0.11658291, 0.02307385)( 0.11758794, 0.02290942)( 0.11859296, 0.02274604)( 0.11959799, 0.02258372)( 0.12060302, 0.02242244)( 0.12160804, 0.02226219)( 0.12261307, 0.02210297)( 0.12361809, 0.02194476)( 0.12462312, 0.02178757)( 0.12562814, 0.02163138)( 0.12663317, 0.02147618)( 0.12763819, 0.02132196)( 0.12864322, 0.02116872)( 0.12964824, 0.02101645)( 0.13065327, 0.02086515)( 0.13165829, 0.02071480)( 0.13266332, 0.02056539)( 0.13366834, 0.02041693)( 0.13467337, 0.02026939)( 0.13567839, 0.02012279)( 0.13668342, 0.01997710)( 0.13768844, 0.01983232)( 0.13869347, 0.01968844)( 0.13969849, 0.01954547)( 0.14070352, 0.01940338)( 0.14170854, 0.01926218)( 0.14271357, 0.01912185)( 0.14371859, 0.01898240)( 0.14472362, 0.01884380)( 0.14572864, 0.01870607)( 0.14673367, 0.01856919)( 0.14773869, 0.01843315)( 0.14874372, 0.01829795)( 0.14974874, 0.01816358)( 0.15075377, 0.01803004)( 0.15175879, 0.01789731)( 0.15276382, 0.01776541)( 0.15376884, 0.01763431)( 0.15477387, 0.01750401)( 0.15577889, 0.01737451)( 0.15678392, 0.01724580)( 0.15778894, 0.01711788)( 0.15879397, 0.01699073)( 0.15979899, 0.01686436)( 0.16080402, 0.01673876)( 0.16180905, 0.01661392)( 0.16281407, 0.01648984)( 0.16381910, 0.01636651)( 0.16482412, 0.01624393)( 0.16582915, 0.01612209)( 0.16683417, 0.01600099)( 0.16783920, 0.01588062)( 0.16884422, 0.01576098)( 0.16984925, 0.01564206)( 0.17085427, 0.01552385)( 0.17185930, 0.01540636)( 0.17286432, 0.01528958)( 0.17386935, 0.01517349)( 0.17487437, 0.01505811)( 0.17587940, 0.01494342)( 0.17688442, 0.01482941)( 0.17788945, 0.01471609)( 0.17889447, 0.01460345)( 0.17989950, 0.01449149)( 0.18090452, 0.01438019)( 0.18190955, 0.01426956)( 0.18291457, 0.01415959)( 0.18391960, 0.01405028)( 0.18492462, 0.01394162)( 0.18592965, 0.01383361)( 0.18693467, 0.01372625)( 0.18793970, 0.01361952)( 0.18894472, 0.01351344)( 0.18994975, 0.01340798)( 0.19095477, 0.01330315)( 0.19195980, 0.01319895)( 0.19296482, 0.01309536)( 0.19396985, 0.01299239)( 0.19497487, 0.01289004)( 0.19597990, 0.01278829)( 0.19698492, 0.01268715)( 0.19798995, 0.01258661)( 0.19899497, 0.01248667)
};
	
\addplot[blue,line width = 1pt] coordinates{
( 0.00100503, 0.00001007)( 0.07738693, 0.00011575)( 0.08140704, 0.00040739)( 0.09246231, 0.00166696)( 0.10150754, 0.00511033)( 0.10954774, 0.01165135)( 0.11356784, 0.01576694)( 0.11959799, 0.02279674)( 0.12864322, 0.03945510)( 0.19798995, 0.17617448)( 0.19899497, 0.17869036)


};

\addplot[red,line width = 1pt,dashed] coordinates{
( 0.004, 0.019)( 0.008, 0.019)( 0.012, 0.019)( 0.016, 0.019)( 0.020, 0.019)( 0.024, 0.019)( 0.029, 0.019)( 0.033, 0.019)( 0.037, 0.019)( 0.041, 0.019)( 0.045, 0.019)( 0.049, 0.019)( 0.053, 0.019)( 0.057, 0.019)( 0.061, 0.019)( 0.065, 0.019)( 0.069, 0.019)( 0.073, 0.019)( 0.078, 0.019)( 0.082, 0.019)( 0.086, 0.019)( 0.090, 0.019)( 0.094, 0.019)( 0.098, 0.019)( 0.102, 0.019)( 0.106, 0.019)( 0.110, 0.019)( 0.114, 0.019)( 0.118, 0.019)( 0.122, 0.019)( 0.127, 0.019)( 0.131, 0.019)( 0.135, 0.019)( 0.139, 0.019)( 0.143, 0.019)( 0.147, 0.019)( 0.151, 0.019)( 0.155, 0.019)( 0.159, 0.019)( 0.163, 0.019)( 0.167, 0.019)( 0.171, 0.019)( 0.176, 0.019)( 0.180, 0.019)( 0.184, 0.019)( 0.188, 0.019)( 0.192, 0.019)( 0.196, 0.019)

};

\addplot[green,line width = 1pt] coordinates{
( 0.001, 0.000)( 0.002, 0.000)( 0.003, 0.000)( 0.004, 0.000)( 0.005, 0.000)( 0.006, 0.000)( 0.007, 0.000)( 0.008, 0.000)( 0.009, 0.000)( 0.010, 0.000)( 0.011, 0.000)( 0.012, 0.000)( 0.013, 0.000)( 0.014, 0.003)( 0.015, 0.007)( 0.016, 0.010)( 0.017, 0.014)( 0.018, 0.017)( 0.019, 0.021)( 0.020, 0.024)( 0.021, 0.027)( 0.022, 0.030)( 0.023, 0.034)( 0.024, 0.037)( 0.025, 0.040)( 0.026, 0.043)( 0.027, 0.046)( 0.028, 0.048)( 0.029, 0.051)( 0.030, 0.054)( 0.031, 0.057)( 0.032, 0.060)( 0.033, 0.062)( 0.034, 0.065)( 0.035, 0.067)( 0.036, 0.070)( 0.037, 0.072)( 0.038, 0.075)( 0.039, 0.077)( 0.040, 0.080)( 0.041, 0.082)( 0.042, 0.085)( 0.043, 0.087)( 0.044, 0.089)( 0.045, 0.092)( 0.046, 0.094)( 0.047, 0.096)( 0.048, 0.098)( 0.049, 0.101)( 0.050, 0.103)( 0.051, 0.105)( 0.052, 0.107)( 0.053, 0.109)( 0.054, 0.111)( 0.055, 0.113)( 0.056, 0.115)( 0.057, 0.117)( 0.058, 0.119)( 0.059, 0.121)( 0.060, 0.123)( 0.061, 0.125)( 0.062, 0.127)( 0.063, 0.129)( 0.064, 0.131)( 0.065, 0.133)( 0.066, 0.135)( 0.067, 0.136)( 0.068, 0.138)( 0.069, 0.140)( 0.070, 0.142)( 0.071, 0.144)( 0.072, 0.145)( 0.073, 0.147)( 0.074, 0.149)( 0.075, 0.151)( 0.076, 0.152)( 0.077, 0.154)( 0.078, 0.156)( 0.079, 0.157)( 0.080, 0.159)( 0.081, 0.161)( 0.082, 0.162)( 0.083, 0.164)( 0.084, 0.166)( 0.085, 0.167)( 0.086, 0.169)( 0.087, 0.170)( 0.088, 0.172)( 0.089, 0.173)( 0.090, 0.175)( 0.091, 0.176)( 0.092, 0.178)( 0.093, 0.179)( 0.094, 0.181)( 0.095, 0.182)( 0.096, 0.184)( 0.097, 0.185)( 0.098, 0.187)( 0.099, 0.188)( 0.101, 0.190)( 0.102, 0.191)( 0.103, 0.192)( 0.104, 0.194)( 0.105, 0.195)( 0.106, 0.197)( 0.107, 0.198)( 0.108, 0.199)( 0.109, 0.201)( 0.110, 0.202)( 0.111, 0.203)( 0.112, 0.205)( 0.113, 0.206)( 0.114, 0.207)( 0.115, 0.209)( 0.116, 0.210)( 0.117, 0.211)( 0.118, 0.212)( 0.119, 0.214)( 0.120, 0.215)( 0.121, 0.216)( 0.122, 0.217)( 0.123, 0.219)( 0.124, 0.220)( 0.125, 0.221)( 0.126, 0.222)( 0.127, 0.224)( 0.128, 0.225)( 0.129, 0.226)( 0.130, 0.227)( 0.131, 0.228)( 0.132, 0.230)( 0.133, 0.231)( 0.134, 0.232)( 0.135, 0.233)( 0.136, 0.234)( 0.137, 0.235)( 0.138, 0.236)( 0.139, 0.238)( 0.140, 0.239)( 0.141, 0.240)( 0.142, 0.241)( 0.143, 0.242)( 0.144, 0.243)( 0.145, 0.244)( 0.146, 0.245)( 0.147, 0.246)( 0.148, 0.247)( 0.149, 0.248)( 0.150, 0.249)( 0.151, 0.250)( 0.152, 0.251)( 0.153, 0.253)( 0.154, 0.254)( 0.155, 0.255)( 0.156, 0.256)( 0.157, 0.257)( 0.158, 0.258)( 0.159, 0.259)( 0.160, 0.260)( 0.161, 0.261)( 0.162, 0.262)( 0.163, 0.263)( 0.164, 0.264)( 0.165, 0.264)( 0.166, 0.265)( 0.167, 0.266)( 0.168, 0.267)( 0.169, 0.268)( 0.170, 0.269)( 0.171, 0.270)( 0.172, 0.271)( 0.173, 0.272)( 0.174, 0.273)( 0.175, 0.274)( 0.176, 0.275)( 0.177, 0.276)( 0.178, 0.277)( 0.179, 0.277)( 0.180, 0.278)( 0.181, 0.279)( 0.182, 0.280)( 0.183, 0.281)( 0.184, 0.282)( 0.185, 0.283)( 0.186, 0.284)( 0.187, 0.284)( 0.188, 0.285)( 0.189, 0.286)( 0.190, 0.287)( 0.191, 0.288)( 0.192, 0.289)( 0.193, 0.289)( 0.194, 0.290)( 0.195, 0.291)( 0.196, 0.292)( 0.197, 0.293)( 0.198, 0.294)( 0.199, 0.294)
};

\addplot[purple,line width = 1pt,dashed] coordinates{
	( 0.004, 0.0529)( 0.008, 0.0529)( 0.012, 0.0529)( 0.016, 0.0529)( 0.020, 0.0529)( 0.024, 0.0529)( 0.029, 0.0529)( 0.033, 0.0529)( 0.037, 0.0529)( 0.041, 0.0529)( 0.045, 0.0529)( 0.049, 0.0529)( 0.053, 0.0529)( 0.057, 0.0529)( 0.061, 0.0529)( 0.065, 0.0529)( 0.069, 0.0529)( 0.073, 0.0529)( 0.078, 0.0529)( 0.082, 0.0529)( 0.086, 0.0529)( 0.090, 0.0529)( 0.094, 0.0529)( 0.098, 0.0529)( 0.102, 0.0529)( 0.106, 0.0529)( 0.110, 0.0529)( 0.114, 0.0529)( 0.118, 0.0529)( 0.122, 0.0529)( 0.127, 0.0529)( 0.131, 0.0529)( 0.135, 0.0529)( 0.139, 0.0529)( 0.143, 0.0529)( 0.147, 0.0529)( 0.151, 0.0529)( 0.155, 0.0529)( 0.159, 0.0529)( 0.163, 0.0529)( 0.167, 0.0529)( 0.171, 0.0529)( 0.176, 0.0529)( 0.180, 0.0529)( 0.184, 0.0529)( 0.188, 0.0529)( 0.192, 0.0529)( 0.196, 0.0529)
	
};

\addplot[mark=*] coordinates {( 0.11959799, 0.02279674)};
\addplot[mark=*] coordinates {( 0.026, 0.043)};

%\addplot[green,line width = 1pt,dashed] coordinates{
%( 0.004, 0.029)( 0.008, 0.029)( 0.012, 0.029)( 0.016, 0.029)( 0.020, 0.029)( 0.024, 0.029)( 0.029, 0.029)( 0.033, 0.029)( 0.037, 0.029)( 0.041, 0.029)( 0.045, 0.029)( 0.049, 0.029)( 0.053, 0.029)( 0.057, 0.029)( 0.061, 0.029)( 0.065, 0.029)( 0.069, 0.029)( 0.073, 0.029)( 0.078, 0.029)( 0.082, 0.029)( 0.086, 0.029)( 0.090, 0.029)( 0.094, 0.029)( 0.098, 0.029)( 0.102, 0.029)( 0.106, 0.029)( 0.110, 0.029)( 0.114, 0.029)( 0.118, 0.029)( 0.122, 0.029)( 0.127, 0.029)( 0.131, 0.029)( 0.135, 0.029)( 0.139, 0.029)( 0.143, 0.029)( 0.147, 0.029)( 0.151, 0.029)( 0.155, 0.029)( 0.159, 0.029)( 0.163, 0.029)( 0.167, 0.029)( 0.171, 0.029)( 0.176, 0.029)( 0.180, 0.029)( 0.184, 0.029)( 0.188, 0.029)( 0.192, 0.029)( 0.196, 0.029)
%};


	\legend{ {hypothesis testing error exponent},{$G$ (Proposition~\ref{Prop:General})},{hypothesis testing without binning},{$\hat{G}$ (Proposition~\ref{Prop:BetterAchievable})},{``Stein'' Upper Bound}}
	\end{axis}
	
	
\end{tikzpicture}

==> Final copy/figures/GaussianEqualMarginals.tex <==
\pgfplotsset{compat=newest}
\pgfkeys{/pgfplots/.cd,master axis/.style={
    scale only axis,
    enlarge x limits=false,
    axis x line*=bottom,
    xticklabel shift=3pt,
    after end axis/.code={
      \pgfkeys{/pgf/fpu=true,/pgf/fpu/output format=fixed}
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmin}}
      \global\let\masterxmin=\pgfmathresult
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmax}}
      \global\let\masterxmax=\pgfmathresult
      \pgfkeys{/pgf/fpu=false}
    },
  },
  slave axis/.style={
    scale only axis,enlarge x limits=false,
    axis x line*=top,
    axis y line=none,
    xmin=\masterxmin,xmax=\masterxmax,
    ymin=0,ymax=0.25,
    scaled x ticks=false,
    xtick={0,0.0457,0.1368,0.2172,0.2858,0.3446,0.3953,0.4394,0.459},
    xticklabels={0.75,0.7,0.6,0.5,0.4,0.3,0.2,0.1,0},
    %  \pgfkeys{/pgf/fpu}%
    %  \pgfmathparse{1/\tick}%
    %  \pgfmathprintnumber{\pgfmathresult}%
    %},
    %  xticklabel style={/pgf/number format/.cd,fixed,precision=2},
    %  xmajorgrids=true, % to show the tick position
    %  every axis x grid/.style={red,dashed,very thick},
  }
}
  % calculation of the xtick position
  %\xdef\slavextick{}
  %\foreach[count=\n][evaluate=\i as \j using 1/\i]%
  % \i in {0.12,0.11,...,0.07} % xtick for the slave axis
  %  {\pgfmathparse{\n==1?"":","}\xdef\slavextick{\slavextick\pgfmathresult\j}
  %  }

\begin{tikzpicture}

\begin{axis}[master axis,
  ymin=0,ymax=0.25,
  xmin=0,xmax=0.459,
  enlarge x limits=false,
  xlabel={$E$},
  ylabel=$D_0$,
]
\addplot[black,line width = 1pt] coordinates{
( 0.008, 0.115)( 0.016, 0.118)( 0.025, 0.121)( 0.033, 0.125)( 0.042, 0.128)( 0.050, 0.131)( 0.059, 0.134)( 0.067, 0.137)( 0.076, 0.140)( 0.084, 0.143)( 0.093, 0.146)( 0.101, 0.149)( 0.109, 0.152)( 0.117, 0.155)( 0.125, 0.158)( 0.133, 0.160)( 0.141, 0.163)( 0.149, 0.166)( 0.156, 0.168)( 0.164, 0.171)( 0.171, 0.173)( 0.178, 0.176)( 0.186, 0.178)( 0.193, 0.181)( 0.200, 0.183)( 0.207, 0.185)( 0.213, 0.188)( 0.220, 0.190)( 0.227, 0.192)( 0.233, 0.194)( 0.240, 0.196)( 0.246, 0.199)( 0.252, 0.201)( 0.258, 0.203)( 0.264, 0.205)( 0.270, 0.207)( 0.276, 0.209)( 0.282, 0.211)( 0.287, 0.213)( 0.293, 0.215)( 0.298, 0.217)( 0.304, 0.218)( 0.309, 0.220)( 0.315, 0.222)( 0.320, 0.224)( 0.325, 0.226)( 0.330, 0.227)( 0.335, 0.229)
};

\addplot[blue,line width = 1pt] coordinates{
( 0.009, 0.031)( 0.018, 0.033)( 0.028, 0.034)( 0.037, 0.035)( 0.047, 0.036)( 0.057, 0.037)( 0.067, 0.038)( 0.077, 0.039)( 0.087, 0.041)( 0.097, 0.042)( 0.107, 0.043)( 0.117, 0.044)( 0.127, 0.045)( 0.137, 0.046)( 0.147, 0.047)( 0.157, 0.048)( 0.166, 0.049)( 0.176, 0.050)( 0.185, 0.051)( 0.195, 0.052)( 0.204, 0.053)( 0.213, 0.055)( 0.222, 0.056)( 0.231, 0.057)( 0.240, 0.058)( 0.249, 0.059)( 0.258, 0.060)( 0.266, 0.061)( 0.275, 0.062)( 0.283, 0.063)( 0.291, 0.064)( 0.300, 0.065)( 0.308, 0.066)( 0.316, 0.067)( 0.324, 0.068)( 0.331, 0.069)( 0.339, 0.070)( 0.347, 0.071)( 0.354, 0.072)( 0.362, 0.073)( 0.369, 0.074)( 0.377, 0.075)( 0.384, 0.075)( 0.391, 0.076)( 0.398, 0.077)( 0.405, 0.078)( 0.412, 0.079)( 0.419, 0.080)
};

\addplot[red,line width = 1pt] coordinates{
( 0.009, 0.008)( 0.019, 0.008)( 0.029, 0.009)( 0.039, 0.009)( 0.049, 0.009)( 0.059, 0.010)( 0.069, 0.010)( 0.080, 0.010)( 0.090, 0.011)( 0.101, 0.011)( 0.111, 0.011)( 0.122, 0.011)( 0.132, 0.012)( 0.142, 0.012)( 0.153, 0.012)( 0.163, 0.013)( 0.173, 0.013)( 0.183, 0.013)( 0.193, 0.014)( 0.203, 0.014)( 0.213, 0.014)( 0.222, 0.015)( 0.232, 0.015)( 0.242, 0.015)( 0.251, 0.015)( 0.260, 0.016)( 0.270, 0.016)( 0.279, 0.016)( 0.288, 0.017)( 0.297, 0.017)( 0.306, 0.017)( 0.314, 0.018)( 0.323, 0.018)( 0.332, 0.018)( 0.340, 0.018)( 0.349, 0.019)( 0.357, 0.019)( 0.365, 0.019)( 0.373, 0.020)( 0.381, 0.020)( 0.389, 0.020)( 0.397, 0.020)( 0.405, 0.021)( 0.413, 0.021)( 0.421, 0.021)( 0.428, 0.022)( 0.436, 0.022)( 0.443, 0.022)
};

\addplot[green,line width = 1pt] coordinates{
( 0.009, 0.001)( 0.019, 0.001)( 0.029, 0.001)( 0.039, 0.001)( 0.049, 0.001)( 0.060, 0.001)( 0.070, 0.001)( 0.081, 0.001)( 0.091, 0.001)( 0.102, 0.001)( 0.113, 0.001)( 0.123, 0.001)( 0.134, 0.001)( 0.144, 0.001)( 0.155, 0.001)( 0.165, 0.001)( 0.175, 0.001)( 0.185, 0.001)( 0.196, 0.001)( 0.206, 0.001)( 0.216, 0.001)( 0.225, 0.001)( 0.235, 0.001)( 0.245, 0.001)( 0.255, 0.001)( 0.264, 0.001)( 0.273, 0.001)( 0.283, 0.001)( 0.292, 0.001)( 0.301, 0.001)( 0.310, 0.001)( 0.319, 0.001)( 0.328, 0.001)( 0.337, 0.001)( 0.346, 0.001)( 0.354, 0.001)( 0.363, 0.001)( 0.371, 0.001)( 0.379, 0.001)( 0.388, 0.001)( 0.396, 0.001)( 0.404, 0.001)( 0.412, 0.001)( 0.420, 0.001)( 0.428, 0.001)( 0.436, 0.001)( 0.443, 0.001)( 0.451, 0.001)
};

\legend{ {$R=1$},{$R=2$},{$R=3$}, {$R=5$}}
\end{axis}

\begin{axis}[slave axis,xlabel=$D_1$]\end{axis}

\end{tikzpicture}

==> Final copy/figures/GaussianSimulation3.tex <==
\pgfplotsset{compat=newest}
\pgfkeys{/pgfplots/.cd,master axis/.style={
    scale only axis,
    enlarge x limits=false,
    axis x line*=bottom,
    xticklabel shift=3pt,
    after end axis/.code={
      \pgfkeys{/pgf/fpu=true,/pgf/fpu/output format=fixed}
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmin}}
      \global\let\masterxmin=\pgfmathresult
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmax}}
      \global\let\masterxmax=\pgfmathresult
      \pgfkeys{/pgf/fpu=false}
    },
  },
  slave axis/.style={
    scale only axis,enlarge x limits=false,
    axis x line*=top,
    axis y line=none,
    xmin=\masterxmin,xmax=\masterxmax,
    ymin=0,ymax=1,
    scaled x ticks=false,
    xtick={0,0.0338,0.0668,0.0976,0.1258,0.1515,0.1750,0.1963,0.2158,0.2336,0.2500},
    xticklabels={2,1.8,1.6,1.4,1.2,1,0.8,0.6,0.4,0.2,0},
    %  \pgfkeys{/pgf/fpu}%
    %  \pgfmathparse{1/\tick}%
    %  \pgfmathprintnumber{\pgfmathresult}%
    %},
    %  xticklabel style={/pgf/number format/.cd,fixed,precision=2},
    %  xmajorgrids=true, % to show the tick position
    %  every axis x grid/.style={red,dashed,very thick},
  }
}
  % calculation of the xtick position
  %\xdef\slavextick{}
  %\foreach[count=\n][evaluate=\i as \j using 1/\i]%
  % \i in {0.12,0.11,...,0.07} % xtick for the slave axis
  %  {\pgfmathparse{\n==1?"":","}\xdef\slavextick{\slavextick\pgfmathresult\j}
  %  }

\begin{tikzpicture}

\begin{axis}[master axis,
  ymin=0,ymax=0.9,
  xmin=0,xmax=0.25,
  enlarge x limits=false,
  xlabel={$E$},
  ylabel=$D_0$,
]
\addplot[black,line width = 1pt] coordinates{
( 0.003, 0.607)( 0.007, 0.614)( 0.010, 0.622)( 0.014, 0.628)( 0.017, 0.635)( 0.021, 0.642)( 0.024, 0.649)( 0.028, 0.655)( 0.031, 0.662)( 0.035, 0.668)( 0.038, 0.674)( 0.041, 0.680)( 0.045, 0.686)( 0.048, 0.692)( 0.052, 0.698)( 0.055, 0.704)( 0.058, 0.710)( 0.062, 0.715)( 0.065, 0.721)( 0.068, 0.726)( 0.071, 0.732)( 0.075, 0.737)( 0.078, 0.742)( 0.081, 0.747)( 0.084, 0.753)( 0.087, 0.758)( 0.090, 0.763)( 0.093, 0.767)( 0.096, 0.772)( 0.099, 0.777)( 0.102, 0.782)( 0.105, 0.786)( 0.108, 0.791)( 0.111, 0.796)( 0.114, 0.800)( 0.117, 0.804)( 0.120, 0.809)( 0.122, 0.813)( 0.125, 0.817)( 0.128, 0.822)( 0.131, 0.826)( 0.133, 0.830)( 0.136, 0.834)( 0.139, 0.838)( 0.141, 0.842)( 0.144, 0.846)( 0.146, 0.850)( 0.149, 0.853)
};

\addplot[blue,line width = 1pt] coordinates{
( 0.004, 0.180)( 0.009, 0.183)( 0.013, 0.186)( 0.018, 0.189)( 0.022, 0.192)( 0.027, 0.195)( 0.031, 0.198)( 0.036, 0.201)( 0.041, 0.204)( 0.045, 0.208)( 0.050, 0.211)( 0.055, 0.214)( 0.060, 0.217)( 0.064, 0.220)( 0.069, 0.222)( 0.074, 0.225)( 0.079, 0.228)( 0.083, 0.231)( 0.088, 0.234)( 0.093, 0.237)( 0.098, 0.240)( 0.102, 0.243)( 0.107, 0.246)( 0.112, 0.249)( 0.116, 0.251)( 0.121, 0.254)( 0.126, 0.257)( 0.130, 0.260)( 0.135, 0.263)( 0.139, 0.265)( 0.144, 0.268)( 0.149, 0.271)( 0.153, 0.274)( 0.158, 0.276)( 0.162, 0.279)( 0.166, 0.282)( 0.171, 0.284)( 0.175, 0.287)( 0.180, 0.290)( 0.184, 0.292)( 0.188, 0.295)( 0.193, 0.298)( 0.197, 0.300)( 0.201, 0.303)( 0.205, 0.306)( 0.209, 0.308)( 0.214, 0.311)( 0.218, 0.313)
};

\addplot[red,line width = 1pt] coordinates{
( 0.004, 0.047)( 0.009, 0.048)( 0.014, 0.049)( 0.019, 0.050)( 0.023, 0.051)( 0.028, 0.052)( 0.033, 0.053)( 0.038, 0.053)( 0.043, 0.054)( 0.048, 0.055)( 0.053, 0.056)( 0.058, 0.057)( 0.064, 0.058)( 0.069, 0.059)( 0.074, 0.060)( 0.079, 0.061)( 0.084, 0.062)( 0.089, 0.062)( 0.094, 0.063)( 0.100, 0.064)( 0.105, 0.065)( 0.110, 0.066)( 0.115, 0.067)( 0.120, 0.068)( 0.125, 0.069)( 0.130, 0.070)( 0.136, 0.070)( 0.141, 0.071)( 0.146, 0.072)( 0.151, 0.073)( 0.156, 0.074)( 0.161, 0.075)( 0.166, 0.076)( 0.171, 0.077)( 0.176, 0.077)( 0.181, 0.078)( 0.186, 0.079)( 0.190, 0.080)( 0.195, 0.081)( 0.200, 0.082)( 0.205, 0.083)( 0.210, 0.084)( 0.215, 0.084)( 0.219, 0.085)( 0.224, 0.086)( 0.229, 0.087)( 0.233, 0.088)( 0.238, 0.089)
};

\addplot[green,line width = 1pt] coordinates{
( 0.005, 0.003)( 0.009, 0.003)( 0.014, 0.003)( 0.019, 0.003)( 0.024, 0.003)( 0.029, 0.003)( 0.034, 0.003)( 0.039, 0.003)( 0.044, 0.003)( 0.049, 0.004)( 0.054, 0.004)( 0.060, 0.004)( 0.065, 0.004)( 0.070, 0.004)( 0.075, 0.004)( 0.081, 0.004)( 0.086, 0.004)( 0.091, 0.004)( 0.097, 0.004)( 0.102, 0.004)( 0.107, 0.004)( 0.112, 0.004)( 0.118, 0.004)( 0.123, 0.004)( 0.128, 0.004)( 0.134, 0.004)( 0.139, 0.005)( 0.144, 0.005)( 0.149, 0.005)( 0.154, 0.005)( 0.160, 0.005)( 0.165, 0.005)( 0.170, 0.005)( 0.175, 0.005)( 0.180, 0.005)( 0.185, 0.005)( 0.190, 0.005)( 0.195, 0.005)( 0.200, 0.005)( 0.205, 0.005)( 0.210, 0.005)( 0.215, 0.005)( 0.220, 0.005)( 0.225, 0.006)( 0.230, 0.006)( 0.235, 0.006)( 0.240, 0.006)( 0.245, 0.006)
};

\legend{ {$R=1$},{$R=2$},{$R=3$}, {$R=5$}}
\end{axis}

\begin{axis}[slave axis,xlabel=$D_1$]\end{axis}

\end{tikzpicture}

==> Final copy/figures/error_distortion_independence.tex <==
\begin{tikzpicture}
	\begin{axis}[
	title = \textbf{},
		xlabel=$E$,
		ylabel=$D\text{[BER]}$,
		xmin = 0,
		ymin = 0,
		xmax = 0.1887,
		ymax = 0.25]
		\pgfplotsset{every axis legend/.append style={
at={(0.98,0.3),font = \small},
anchor= south east}}



%	\addplot[blue,line width=1pt] coordinates {
%(0.500,0.681) (0.600,0.615) (0.700,0.566) (0.800,0.529) (0.900,0.499) (1.000,0.475) (1.100,0.455) (1.200,0.438) (1.300,0.424) (1.400,0.411) (1.500,0.401) (1.600,0.391) (1.700,0.383) (1.800,0.375) (1.900,0.368) (2.000,0.362) (2.100,0.357) (2.200,0.352) (2.300,0.347) (2.400,0.343) 
%	};
%	
%	\addplot[red,line width=1pt] coordinates {
%(0.500,0.613) (0.600,0.543) (0.700,0.491) (0.800,0.452) (0.900,0.421) (1.000,0.396) (1.100,0.375) (1.200,0.358) (1.300,0.343) (1.400,0.330) (1.500,0.319) (1.600,0.310) (1.700,0.301) (1.800,0.294) (1.900,0.287) (2.000,0.281) (2.100,0.275) (2.200,0.270) (2.300,0.266) (2.400,0.261) 
%	};
	
%	\addplot[black,dotted,line width=1pt] coordinates {
%(1.100,0.346) (1.200,0.329) (1.300,0.314) (1.400,0.301) (1.500,0.289) (1.600,0.278) (1.700,0.268) (1.800,0.260) (1.900,0.252) (2.000,0.244) (2.100,0.238) (2.200,0.231) (2.300,0.226) (2.400,0.220) (2.500,0.215) (2.600,0.211) (2.700,0.206) (2.800,0.202) (2.900,0.199) (3.000,0.195) 
%	};

\addplot[black,line width = 1pt] coordinates{
( 0.000, 0.214)( 0.010, 0.217)( 0.020, 0.221)( 0.030, 0.224)( 0.040, 0.228)( 0.050, 0.232)( 0.060, 0.235)( 0.070, 0.239)( 0.080, 0.243)( 0.090, 0.247)( 0.100, 0.250)
};
	
\addplot[blue,line width = 1pt] coordinates{
( 0.000, 0.177)( 0.019, 0.184)( 0.038, 0.191)( 0.057, 0.198)( 0.075, 0.205)( 0.094, 0.211)( 0.113, 0.218)( 0.132, 0.225)( 0.151, 0.232)( 0.170, 0.239)( 0.189, 0.246)
};

\addplot[red,line width = 1pt] coordinates{
( 0.000, 0.069)( 0.019, 0.075)( 0.038, 0.082)( 0.057, 0.088)( 0.075, 0.095)( 0.094, 0.102)( 0.113, 0.109)( 0.132, 0.116)( 0.151, 0.123)( 0.170, 0.130)( 0.189, 0.136)
};

\addplot[green,line width = 1pt] coordinates{
( 0.000, 0.001)( 0.019, 0.006)( 0.038, 0.008)( 0.057, 0.011)( 0.075, 0.014)( 0.094, 0.017)( 0.113, 0.021)( 0.132, 0.025)( 0.151, 0.029)( 0.170, 0.033)( 0.189, 0.037)
};

\addplot[orange,line width = 1pt] coordinates{
( 0.000, 0.000)( 0.019, 0.000)( 0.038, 0.000)( 0.057, 0.000)( 0.075, 0.000)( 0.094, 0.000)( 0.113, 0.005)( 0.132, 0.007)( 0.151, 0.010)( 0.170, 0.013)( 0.189, 0.016)
};

\addplot[purple,line width = 1pt] coordinates{
( 0.000, 0.000)( 0.019, 0.000)( 0.038, 0.000)( 0.057, 0.000)( 0.075, 0.000)( 0.094, 0.000)( 0.113, 0.000)( 0.132, 0.000)( 0.151, 0.000)( 0.170, 0.000)( 0.189, 0.000)

};

	\legend{ {$R=0.1$},{$R=0.2$},{$R=0.5$}, {$R=0.8$},{$R=0.9$},{$R=1$}}
	\end{axis}
	
	
\end{tikzpicture}

==> Final copy/packages-2.tex <==

%--------------------------------------------------------------------
% packages standards
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{times}
\usepackage{graphicx}
\usepackage{color}
\usepackage{verbatim}
\usepackage{cite}

%--------------------------------------------------------------------
% autres packages

% pour les figures
\usepackage{subfig}		
%\usepackage{pgf}		
%\usepackage{tikz}
%\usepackage{pgfplots}	
%\usetikzlibrary{decorations}
%\usetikzlibrary{patterns}
%\usetikzlibrary{positioning}
%\usetikzlibrary{backgrounds}
%\usetikzlibrary{fit}
%\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{shapes.symbols}
%\usetikzlibrary{calc}

%--------------------------------------------------------------------
% pour passer temporairement en paysage
% \usepackage{pdflscape}
% \usepackage{lscape}

%--------------------------------------------------------------------
% pour \minuso
\usepackage{stmaryrd}

%--------------------------------------------------------------------
% pour barrer ie, simplifier des termes
\usepackage{cancel}
\usepackage[normalem]{ulem}

%--------------------------------------------------------------------
% pour commenter des blocs
\usepackage{verbatim}

%--------------------------------------------------------------------
\newtheorem{definition}	{Definition}
\newtheorem{theorem}	{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}		{Lemma}
\newtheorem{corollary}	{Corollary}
\newtheorem{remark}		{Remark}


==> Final copy/packages.tex <==

%--------------------------------------------------------------------
% packages standards
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{times}
\usepackage{graphicx}
\usepackage{color}
\usepackage{verbatim}
\usepackage{cite}

%--------------------------------------------------------------------
% autres packages

% pour les figures
\usepackage{subfig}		
%\usepackage{pgf}		
%\usepackage{tikz}
%\usepackage{pgfplots}	
%\usetikzlibrary{decorations}
%\usetikzlibrary{patterns}
%\usetikzlibrary{positioning}
%\usetikzlibrary{backgrounds}
%\usetikzlibrary{fit}
%\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{shapes.symbols}
%\usetikzlibrary{calc}

%--------------------------------------------------------------------
% pour passer temporairement en paysage
% \usepackage{pdflscape}
% \usepackage{lscape}

%--------------------------------------------------------------------
% pour \minuso
\usepackage{stmaryrd}

%--------------------------------------------------------------------
% pour barrer ie, simplifier des termes
\usepackage{cancel}
\usepackage[normalem]{ulem}

%--------------------------------------------------------------------
% pour commenter des blocs
\usepackage{verbatim}

%--------------------------------------------------------------------
\newtheorem{definition}	{Definition}
\newtheorem{theorem}	{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}		{Lemma}
\newtheorem{corollary}	{Corollary}
\newtheorem{remark}		{Remark}


==> commandes-2.tex <==


%--------------------------------------------------------------------
% ensembles
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\sE}{{\mathsf E}}

%\newcommand{\bP}{{\mathbb P}}
\newcommand{\bN}{{\mathbb N}}
\newcommand{\bC}{{\mathbb C}}
\newcommand{\bR}{{\mathbb R}}
\newcommand{\bZ}{{\mathbb Z}}

\newcommand{\sX}{{\mathsf X}}
\newcommand{\sY}{{\mathsf Y}}
\newcommand{\sS}{{\mathsf S}}
\newcommand{\snr}{{\textrm{snr}}}


%------------------------------------------------------------------------------
% intervalles FR [a;b], (a;b], [a;b) ou (a;b)
\newcommand{\intervalFR}[4]{\mathopen{#1}#2\mathclose{}\mathpunct{};#3\mathclose{#4}}
\newcommand{\intervalFRLR}[4]{\left #1 #2\mathpunct{};#3\right #4}

% intervalles ISO 31-11 [a,b], (a,b], [a,b) ou (a,b)
\newcommand{\interval}[4]{\mathopen{#1}#2\mathclose{},#3\mathclose{#4}}
\newcommand{\intervalLR}[4]{\left #1 #2,#3\right #4}

\newcommand{\intFF}[2]{\interval{[}{#1}{#2}{]}}
\newcommand{\intOF}[2]{\interval{(}{#1}{#2}{]}}
\newcommand{\intFO}[2]{\interval{[}{#1}{#2}{)}}
\newcommand{\intOO}[2]{\interval{(}{#1}{#2}{)}}

\newcommand{\intFFLR}[2]{\intervalLR{[}{#1}{#2}{]}}
\newcommand{\intOFLR}[2]{\intervalLR{(}{#1}{#2}{]}}
\newcommand{\intFOLR}[2]{\intervalLR{[}{#1}{#2}{)}}
\newcommand{\intOOLR}[2]{\intervalLR{(}{#1}{#2}{)}}


%------------------------------------------------------------------------------ 
% probabilité
\newcommand{\pr}[1]{\operatorname{Pr}\left\{#1\right\}}

% proba et espérance
\newcommand{\bE}{{\mathbb E}}
\newcommand{\bP}{{\mathbb P}}

% variance Var[.]
\newcommand{\Var}[1]{\text{Var}\left[#1\right]}

% variables aléatoires indépendantes
\newcommand{\indpt}{\perp\!\!\!\perp}

% chaîne de Markov
\newcommand{\mkv}{-\!\!\!\!\minuso\!\!\!\!-}

% relation d'ordre pour "less noisy"
\newcommand{\lessnoisy}[1]{\succeq_{\scriptscriptstyle #1}}

% ensemble typique
\newcommand{\typ}[2]{T_\delta^{#1}(#2)}

% barre au-dessus du texte pour exprimer l'événement complémentaire
\newcommand{\non}[1]{\stackrel{\_\_\_\_\_}{\text{#1}}}

% \sim pour variables i.i.d.
\newcommand{\simiid}{\stackrel{\text{i.i.d.}}{\sim}}

% loi uniforme sur un ensemble, loi de Bernoulli 
\newcommand{\unif}[1]{{\mathcal U}_{\,#1}}
\newcommand{\bern}{{\mathcal B}}

% loi normale
\newcommand{\cN}{{\mathcal N}}


%------------------------------------------------------------------------------
% transposée
\newcommand{\T}{^\text{\scshape{t}}}

%------------------------------------------------------------------------------
% norme et valeur absolue
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}


%------------------------------------------------------------------------------
% limite -> quand (.) tend vers (.)
\newcommand{\toas}[1]{\xrightarrow[#1]{}}


%------------------------------------------------------------------------------
% événement d'erreur
\newcommand{\err}{{\mathsf E}}
\newcommand{\Nerr}{\cancel{\mathsf E}}


%------------------------------------------------------------------------------
% indicatrice
\newcommand{\ind}[1]{\mathbf{1}_{#1}}


%------------------------------------------------------------------------------
% parties entières
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


==> commandes.tex <==


%--------------------------------------------------------------------
% ensembles
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

\newcommand{\sE}{{\mathsf E}}

%\newcommand{\bP}{{\mathbb P}}
\newcommand{\bN}{{\mathbb N}}
\newcommand{\bC}{{\mathbb C}}
\newcommand{\bR}{{\mathbb R}}
\newcommand{\bZ}{{\mathbb Z}}

\newcommand{\sX}{{\mathsf X}}
\newcommand{\sY}{{\mathsf Y}}
\newcommand{\sS}{{\mathsf S}}
\newcommand{\snr}{{\textrm{snr}}}


%------------------------------------------------------------------------------
% intervalles FR [a;b], (a;b], [a;b) ou (a;b)
\newcommand{\intervalFR}[4]{\mathopen{#1}#2\mathclose{}\mathpunct{};#3\mathclose{#4}}
\newcommand{\intervalFRLR}[4]{\left #1 #2\mathpunct{};#3\right #4}

% intervalles ISO 31-11 [a,b], (a,b], [a,b) ou (a,b)
\newcommand{\interval}[4]{\mathopen{#1}#2\mathclose{},#3\mathclose{#4}}
\newcommand{\intervalLR}[4]{\left #1 #2,#3\right #4}

\newcommand{\intFF}[2]{\interval{[}{#1}{#2}{]}}
\newcommand{\intOF}[2]{\interval{(}{#1}{#2}{]}}
\newcommand{\intFO}[2]{\interval{[}{#1}{#2}{)}}
\newcommand{\intOO}[2]{\interval{(}{#1}{#2}{)}}

\newcommand{\intFFLR}[2]{\intervalLR{[}{#1}{#2}{]}}
\newcommand{\intOFLR}[2]{\intervalLR{(}{#1}{#2}{]}}
\newcommand{\intFOLR}[2]{\intervalLR{[}{#1}{#2}{)}}
\newcommand{\intOOLR}[2]{\intervalLR{(}{#1}{#2}{)}}


%------------------------------------------------------------------------------ 
% probabilité
\newcommand{\pr}[1]{\operatorname{Pr}\left\{#1\right\}}

% proba et espérance
\newcommand{\bE}{{\mathbb E}}
\newcommand{\bP}{{\mathbb P}}

% variance Var[.]
\newcommand{\Var}[1]{\text{Var}\left[#1\right]}

% variables aléatoires indépendantes
\newcommand{\indpt}{\perp\!\!\!\perp}

% chaîne de Markov
\newcommand{\mkv}{-\!\!\!\!\minuso\!\!\!\!-}

% relation d'ordre pour "less noisy"
\newcommand{\lessnoisy}[1]{\succeq_{\scriptscriptstyle #1}}

% ensemble typique
\newcommand{\typ}[2]{T_\delta^{#1}(#2)}

% barre au-dessus du texte pour exprimer l'événement complémentaire
\newcommand{\non}[1]{\stackrel{\_\_\_\_\_}{\text{#1}}}

% \sim pour variables i.i.d.
\newcommand{\simiid}{\stackrel{\text{i.i.d.}}{\sim}}

% loi uniforme sur un ensemble, loi de Bernoulli 
\newcommand{\unif}[1]{{\mathcal U}_{\,#1}}
\newcommand{\bern}{{\mathcal B}}

% loi normale
\newcommand{\cN}{{\mathcal N}}


%------------------------------------------------------------------------------
% transposée
\newcommand{\T}{^\text{\scshape{t}}}

%------------------------------------------------------------------------------
% norme et valeur absolue
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}


%------------------------------------------------------------------------------
% limite -> quand (.) tend vers (.)
\newcommand{\toas}[1]{\xrightarrow[#1]{}}


%------------------------------------------------------------------------------
% événement d'erreur
\newcommand{\err}{{\mathsf E}}
\newcommand{\Nerr}{\cancel{\mathsf E}}


%------------------------------------------------------------------------------
% indicatrice
\newcommand{\ind}[1]{\mathbf{1}_{#1}}


%------------------------------------------------------------------------------
% parties entières
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}


==> defintions.tex <==

 \section{Strongly typical sequences and related results}
  \label{app:strongly}
  In this appendix we introduce standard notions in information theory but suited for the mathematical developments and proof needed in this work. The results presents can be easily derived from the standard formulations provided in~\cite{ELGamal-Kim-book} and~\cite{Csiszar81}. Be $\mathcal{X}$ and $\mathcal{Y} $  finite alphabets and $(x^n,y^n)\in\mathcal{X}^n\times \mathcal{Y}^n$.  With $\mathcal{P}(\mathcal{X}\times \mathcal{Y})$ we denote the set of all probability distributions on $\mathcal{X}\times\mathcal{Y}$. We define the \emph{strongly $\delta$-typical} sets as:
 
 \begin{definition}[Strongly typical set]
 Consider $p\in\mathcal{P}(\mathcal{X})$ and $\delta>0$. We say that $x^n\in\mathcal{X}^n$ is $p\delta$- strongly typical if $x^n\in\mathcal{T}_{[p]\delta}^n$ with:
 \begin{equation}
 \mathcal{T}_{[p]\delta}^n=\left\{x^n\in\mathcal{X}^n:\Big|\frac{N(a|x^n)}{n}-p(a)\Big|\leq\frac{\delta}{\|\mathcal{X}\|},\ \forall a\in\mathcal{X}\ \mbox{such that}\ p(a)\neq 0\right\}\ ,
 \label{eq:strong_delta_typ}
 \end{equation}
 where $N(a|x^n)$ denotes de number of occurrences of $a\in\mathcal{X}$ in $x^n$ and $p\in\mathcal{P}(\mathcal{X})$.  When $X\sim p_X(x)$ we can denote the corresponding set of strongly typical sequences as $\mathcal{T}_{[X]\delta}^n$. 
  \end{definition}
 Similarly, given $p_{XY}\in\mathcal{P}\left(\mathcal{X}\times\mathcal{Y}\right)$ we can construct the set of $\delta$-jointly typical sequences as:
  \begin{gather}
  \mathcal{T}_{[XY]\delta}^n=\left\{(x^n,y^n)\in\mathcal{X}^n\times\mathcal{Y}^n:\Big|\frac{N(a,b|x^n,y^n)}{n}-p_{XY}(a,b)\Big|\leq\frac{\delta}{\|\mathcal{X}\|\|\mathcal{Y}\|},\right.\nonumber\\
  \left.\ \forall (a,b)\in\mathcal{X}\times\mathcal{Y}\ \mbox{such that}\ p_{XY}(a,b)\neq 0\right\}\ .
  \label{eq:joint_strong_delta_typ}
  \end{gather}
 We also define the \emph{conditional} typical sequences. In precise terms, given $x^n\in\mathcal{X}^n$ we consider the set:
 \begin{gather}
 \mathcal{T}_{[Y|X]\delta}^n(x^n)=\Big\{y^n\in\mathcal{Y}^n:\Big|\frac{N(a,b|x^n,y^n)}{n}-p_{XY}(a,b)\Big|\leq\frac{\delta}{\|\mathcal{X}\|\|\mathcal{Y}\|},\nonumber\\
\ \forall (a,b)\in\mathcal{X}\times\mathcal{Y}\ \mbox{such that}\ p_{XY}(a,b)\neq 0\Big\}\ .
\label{eq:cond_strong_delta_typ}
 \end{gather} 
 Notice that we the following is an alternative writing of this set:
 \begin{equation} 
 \mathcal{T}_{[Y|X]\delta}^n(x^n)=\left\{y^n\in\mathcal{Y}^n:(x^n,y^n)\in\mathcal{T}_{[XY]\delta}^n\right\} \ .
 \end{equation}
 
 We have several useful and standard lemmas, which will be presented without proof (except for the last one):
 
 \begin{lemma}[Properties of typical sets~\cite{Csiszar81}] 
 The following are true:
 \begin{enumerate}
 \item  Consider $(x^n,y^n)\in\mathcal{T}_{[XY]\epsilon}^n$. Then, $x^n\in\mathcal{T}_{[X]\epsilon}^n$, $y^n\in\mathcal{T}_{[Y]\epsilon}$, $x^n\in\mathcal{T}_{[X|Y]\epsilon}^n(y^n)$ and $y^n\in\mathcal{T}_{[Y|X]\epsilon}^n(x^n)$ \ .
 \item Be $T_{[Y|X]\epsilon}^n(x^n)$ with $x^n\notin\mathcal{T}^n_{[X]\epsilon}$. Then $T_{[Y|X]\epsilon}^n(x^n)=\varnothing$ \ .
 \item Be $(X^n,Y^n)\sim\prod_{t=1}^np_{XY}(x_t,y_t)$. If $x^n\in\mathcal{T}_{[X]\epsilon}^n$ we have
 \[2^{-n(H(X)+\delta(\epsilon))}\leq p_{X^n}(x^n)\leq 2^{-n(H(X)-\delta(\epsilon))} \]
 with $\delta(\epsilon)\rightarrow 0$ when $\epsilon\rightarrow 0$. Similarly, if $y^n\in\mathcal{T}_{[Y|X]\epsilon}^n(x^n)$:
  \[2^{-n(H(Y|X)+\delta'(\epsilon))}\leq p_{Y^n|X^n}(y^n|x^n)\leq 2^{-n(H(Y|X)-\delta'(\epsilon))} \]
  with $\delta'(\epsilon)\rightarrow 0$ when $\epsilon\rightarrow 0$\ .
 \label{lemma:cont}
 \end{enumerate}
 \label{lemma:useful}
 \end{lemma}
 
 \begin{lemma}[Conditional typicality lemma~\cite{Csiszar81}]
 Consider de product measure $\prod_{t=1}^np_{XY}(x_t,y_t)$. Using that measure, we have the following 
 \[\operatorname{Pr}\left\{\mathcal{T}_{[X]\epsilon}^n\right\}\geq 1-\mathcal{O}\left(c_1^{-nf(\epsilon)}\right),\ \ c_1>1\]
 where $f(\epsilon)\rightarrow 0$ when $\epsilon\rightarrow 0$. In addition, for every  $x^n\in\mathcal{T}^n_{[X]\epsilon'}$ with $\epsilon'<\frac{\epsilon}{\|\mathcal{Y}\|}$ we have:
 \[\operatorname{Pr}\left\{\mathcal{T}_{[Y|X]\epsilon}^n(x^n)|x^n\right\}\geq 1-\mathcal{O}\left(c_2^{-ng(\epsilon,\epsilon')}\right),\ \ c_2>1\]
 where $g(\epsilon,\epsilon')\rightarrow 0$ when $\epsilon,\epsilon'\rightarrow 0$.
 \label{lemma:prob_lim}
 \end{lemma}
 
 \begin{lemma}[Size of typical sets~\cite{Csiszar81}]
Given $p_{XY}\in\mathcal{P}\left(\mathcal{X}\times\mathcal{Y}\right)$ we have
  \[\frac{1}{n}\|\mathcal{T}_{[X]\epsilon}^n\|\leq H(X)+\delta(\epsilon),\ \  \frac{1}{n}\|\mathcal{T}_{[X]\epsilon}^n\|\geq H(X)-\delta'(\epsilon,n)\]
  where $\delta(\epsilon),\delta'(\epsilon,n)\rightarrow 0$ when $\epsilon\rightarrow 0$ and $n\rightarrow\infty$. Similarly for every $x^n\in\mathcal{X}^n$ we have:
  \[\frac{1}{n}\|\mathcal{T}_{[Y|X]\epsilon}^n(x^n)\|\leq H(Y|X)+\delta(\epsilon)\]
  with $\delta(\epsilon)\rightarrow 0$ with $\epsilon\rightarrow 0$. In addition, for every $x^n\in\mathcal{T}_{[X]\epsilon'}^n$ with $\epsilon'<\frac{\epsilon}{\|\mathcal{Y}\|}$ we have:
    \[\frac{1}{n}\|\mathcal{T}_{[Y|X]\epsilon}^n(x^n)\|\geq H(Y|X)-\delta'(\epsilon,\epsilon',n)\]
 where $\delta'(\epsilon,\epsilon',n)\rightarrow 0$ when $\epsilon,\epsilon'\rightarrow 0$ and $n\rightarrow\infty$.
 \label{lemma:size}
 \end{lemma}
 
 \begin{lemma}[Joint typicality lemma~\cite{Csiszar81}]
 \label{lemma:joint_typ_strong}
 Consider $(X,Y,Z)\sim p_{XYZ}(x,y,z)$ and $(x^n,y^n)\in\mathcal{T}_{[XY]\epsilon'}^n$ with $\epsilon'<\frac{\epsilon}{\|\mathcal{Z}\|}$ and $\epsilon<\epsilon''$. If $p_{Z^n|X^n}(z^n|x^n)=\frac{\mathds{1}\left\{z^n\in\mathcal{T}_{[Z|X]\epsilon''}^n(x^n)\right\}}{\|\mathcal{T}_{[Z|X]\epsilon''}(x^n)\|}$ there exists $\delta'(\epsilon,\epsilon',\epsilon'',n)$ which goes to zero  as $\epsilon,\epsilon',\epsilon''\rightarrow 0$ and $n\rightarrow\infty$ and: 
 \[2^{-n(I(Y;Z|X)+\delta')}\leq\operatorname{Pr}\left\{\tilde{Z}^n\in\mathcal{T}_{[Z|XY]\epsilon}^n(x^n,y^n)\right\}\leq 2^{-n(I(Y;Z|X)-\delta')}\]
 \end{lemma}

\begin{lemma}[Covering Lemma~\cite{ELGamal-Kim-book}]
\label{lemma:covering}
Be $(U,V,X)\sim p_{UVX}$ and $(x^n,u^n)\in\mathcal{T}_{[XU]\epsilon'}^n$, $\epsilon'<\frac{\epsilon}{\|\mathcal{V}\|}$ and $\epsilon<\epsilon''$. Consider also $\left\{V^n(m)\right\}_{m=1}^{2^{nR}}$ random vectors  which are independently generated according to $\frac{\mathds{1}\left\{v^n\in\mathcal{T}_{[V|U]\epsilon''}^n(u^n)\right\}}{\|\mathcal{T}_{[V|U]\epsilon''}(u^n)\|}$. Then:
\begin{equation}
\mbox{Pr}\left\{V^n(m)\notin\mathcal{T}_{[V|UX]\epsilon}^n(x^n,u^n)\ \mbox{for all}\ m\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
uniformly for every  $(x^n,u^n)\in\mathcal{T}^n_{[XU]\epsilon'}$  if: 
\begin{equation}
R>I\left(V;X|U\right)+\delta(\epsilon,\epsilon',\epsilon'',n)
\label{eq:covering_lemma}
\end{equation}
where $\delta(\epsilon,\epsilon',\epsilon'',n)\rightarrow 0$ when $\epsilon,\epsilon',\epsilon''\rightarrow 0$ and $n\rightarrow \infty$.
\end{lemma}
\begin{corollary}
\label{coro:covering}
Assume the conditions in Lemma~\ref{lemma:covering}, and  also:
\begin{equation}
\mbox{Pr}\left\{\left(X^n,U^n\right)\in\mathcal{T}^n_{[XU]\epsilon'}\right\}\xrightarrow[n\rightarrow\infty]{}1\ .
\end{equation}
Then:
\begin{equation}
\mbox{Pr}\left\{\left(U^n,X^n,V^n(m))\right)\notin\mathcal{T}_{[UXV]\epsilon}^n\ \mbox{for all}\ m\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
when (\ref{eq:covering_lemma}) is satisfied.
\end{corollary}

\begin{lemma}[Packing Lemma~\cite{ELGamal-Kim-book}]
\label{lemma:packing}
Be $(U_1U_2WV_1V_2X)\sim p_{U_1U_2WV_1V_2X}$, $(x^n,w^n,v_1^n,v_2^n)\in\mathcal{T}^n_{[XWV_1V_2]\epsilon'}$ and  $\epsilon'<\frac{\epsilon}{\|\mathcal{U}_1\|\|\mathcal{U}_2\|}$ and $\epsilon<\min{\left\{\epsilon_1,\epsilon_2\right\}}$. Consider random vectors $\left\{U_1^n(m_1)\right\}_{m_1=1}^{\mathcal{A}_1}$ and $\left\{U_2^n(m_2)\right\}_{m_2=1}^{\mathcal{A}_2}$ which are independently generated according to 
\begin{equation*}
\frac{\mathds{1}\left\{u_i^n\in\mathcal{T}_{[U_i|V_iW]\epsilon_i}^n(v_i^n,w^n)\right\}}{\|\mathcal{T}_{[U_i|V_iW]\epsilon_i}(w^n,v_i^n)\|},\ i=1,2\ ,
\end{equation*}
and $\mathcal{A}_1,\mathcal{A}_2$ are positive random variables independent of everything else. Then
\begin{equation}
\mbox{Pr}\left\{\left(U_1^n(m_1),U_2^n(m_2)\right)\in\mathcal{T}_{[U_1U_1|XWV_1V_2]\epsilon}^n(x^n,w^n,v_1^n,v_2^n)\ \mbox{for some}\ (m_1,m_2)\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
uniformly for every  $(x^n,w^n,v_1^n,v_2^n)\in\mathcal{T}^n_{[XWV_1V_2]\epsilon'}$  provided that: 

\begin{equation}
\frac{\log{\mathbb{E}\left[\mathcal{A}_1\mathcal{A}_2\right]}}{n}<I\left(U_1;XV_2U_2|WV_1\right)+I\left(U_2;XV_1U_1|WV_2\right)-I\left(U_1;U_2|XWV_1V_2\right)-\delta
\label{eq:packing_lemma}
\end{equation}
where $\delta\equiv\delta(\epsilon,\epsilon',\epsilon_1,\epsilon_2,n)\rightarrow 0$ when $\epsilon,\epsilon',\epsilon_1,\epsilon_2\rightarrow 0$ and $n\rightarrow \infty$.
\end{lemma}

\begin{corollary}
\label{coro:packing}
Assume the conditions in Lemma~\ref{lemma:packing}, and  also:
\begin{equation}
\mbox{Pr}\left\{\left(X^n,W^n,V_1^n,V_2^n\right)\in\mathcal{T}^n_{[XWV_1V_2]\epsilon'}\right\}\xrightarrow[n\rightarrow\infty]{}1
\end{equation}
Then:
\begin{equation}
\mbox{Pr}\left\{\left(U_1^n(m_1),U_2^n(m_2),X^n,W^n,V_1^n,V_2^n)\right)\in\mathcal{T}_{[U_1U_1XWV_1V_2]\epsilon}^n\ \mbox{for some}\ (m_1,m_2)\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
when (\ref{eq:packing_lemma}) is satisfied.
\end{corollary}

\begin{lemma}[Generalized Markov Lemma~\cite{GML_ours_2014} ]
Consider a pmf $p_{UXY}$ belonging to $\mathcal{P}\left(\mathcal{X}\times\mathcal{Y}\times\mathcal{U}\right)$ and that satisfies de following:
\[Y\mkv X\mkv U\]
Consider $(x^n,y^n)\in\mathcal{T}^n_{[XY]\epsilon'}$ and random vectors $U^n$  generated according to:

\begin{equation}
\label{eq:u_dist}
\mbox{Pr}\left\{U^n=u^n\Big|x^n,y^n,U^n\in\mathcal{T}^n_{[U|X]\epsilon''}(x^n)\right\}=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|X]\epsilon''}^n(x^n)\right\}}{\|\mathcal{T}_{[U|X]\epsilon''}^n(x^n)\|}
\end{equation}
For sufficiently small $\epsilon,\epsilon',\epsilon''$ the following holds uniformly for every  $(x^n,y^n)\in\mathcal{T}^n_{[XY]\epsilon'}$:

\begin{equation}
\mbox{Pr}\left\{U^n\notin\mathcal{T}^n_{[U|XY]\epsilon}(x^n,y^n)\Big|x^n,y^n,U^n\in\mathcal{T}^n_{[U|X]\epsilon''}(x^n)\right\}=\mathcal{O}\left(c^{-n}\right)
\end{equation}
where $c>1$.
  \label{lemma:markov}
  \end{lemma}

%  \begin{lemma}[Markov Lemma]
%Consider a pmf $p_{UVXYZ}$ on a finite product alphabet $\mathcal{X}\times\mathcal{Y}\times\mathcal{Z}\times\mathcal{U}\times\mathcal{V}$ and that satifies de following:
%\[(UXZ)\mkv Y\mkv V,\ \ (VYZ)\mkv X\mkv U\]
%Consider $(x^n,y^n,z^n)\in\mathcal{T}^n_{[XYZ]\delta}$ and random vectors $U^n$ and $V^n$ generated according to:
%\[p_{U^nV^n|X^nY^nZ^n}(u^n,v^n|x^n,y^n,z^n)=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|X]\delta}^n(x^n)\right\}}{\|\mathcal{T}_{[U|X]\delta}^n(x^n)\|}\frac{\mathds{1}\left\{v^n\in\mathcal{T}_{[V|Y]\delta}^n(y^n)\right\}}{\|\mathcal{T}_{[V|Y]\delta}^n(y^n)\|}\]
%For sufficiently small $\delta$ and $\epsilon$ the following holds:
%\[\mbox{Pr}\left\{(U^n,V^n)\notin\mathcal{T}^n_{[UV|XYZ]\epsilon}(x^n,y^n,z^n)|x^n,y^n,z^n\right\}=\mathcal{O}\left(c^{-n}\right)\]
%where $c>1$.
%  \label{lemma:markov}
%  \end{lemma}
\begin{corollary}
\label{coro:markov}
Assume the conditions in Lemma~\ref{lemma:markov}, and also:
\begin{equation}
\mbox{Pr}\left\{\left(X^n,Y^n\right)\in\mathcal{T}^n_{[XY]\epsilon'}\right\}\xrightarrow[n\rightarrow\infty]{}1
\end{equation}
and that uniformly for every $(x^n,y^n)\in\mathcal{T}^n_{[XY]\epsilon'}$:
\begin{equation}
\mbox{Pr}\left\{U^n\notin\mathcal{T}^n_{[U|X]\epsilon''}(x^n)\Big| x^n,y^n\right\}\xrightarrow[n\rightarrow\infty]{}0
\end{equation}
we obtain:
\begin{equation}
\mbox{Pr}\left\{(U^n,X^n,Y^n)\in\mathcal{T}^n_{[UXY]\epsilon}\right\}\xrightarrow[n\rightarrow\infty]{}1\ .
\end{equation}
\end{corollary}
 Lemma~\ref{lemma:markov} and Corollary~\ref{coro:markov} will be central for us. They will guarantee the joint typicality of the descriptions generated in different encoders considering the pmf of the chosen descriptions induced by the coding scheme used. 
 %See the differences with lemma \ref{lemma:prob_lim}. In fact, Markov lemma is more useful that \ref{lemma:prob_lim}, where the random vectors $U^n$ are generated through the product measure $\prod_{i=1}^np_{U|XY}(u_i|x_iy_i)=\prod_{i=1}^np_{U|X}(u_i|x_i)$. ç
 The original proof of this result is given in~\cite{PhD-Tung} and involves a combination of rather sophisticated algebraic and combinatorial arguments over finite alphabets. Alternative  proof was also provided  in~\cite{ELGamal-Kim-book}, 
 \begin{equation}
 \mbox{Pr}\left\{(U^nX^n,Y^n)\in\mathcal{T}^n_{[UXY]\epsilon}\right\}\xrightarrow[n\rightarrow\infty]{}1
 \end{equation}
which strongly relies on a rather obscure result by Uhlmann~\cite{Uhlmann} on combinatorics. In~\cite{GML_ours_2014} a short and more general proof of this result is given.

We next present a result which will be useful for proving theorem  \ref{theo-main-theorem}. In order to use the Markov lemma we need to show that the descriptions induced by the encoding procedure in each node satisfies (\ref{eq:u_dist}).
   \begin{lemma}[Encoding induced distribution]   \label{lemma:induced}
 Consider a pmf $p_{UXW}$ belonging to $\mathcal{P}\left(\mathcal{U}\times\mathcal{X}\times\mathcal{W}\right)$ and $\epsilon'\geq\epsilon$.  Be $\left\{U^n(m)\right\}_{m=1}^{S}$ random vectors independently generated according to 
 $$
 \frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|W]\epsilon'}^n(w^n)\right\}}{\|\mathcal{T}_{[U|W]\epsilon'}(w^n)\|}
 $$ 
 and where $(W^n,X^n)$ are generated with an arbitrary distribution. Once these vectors are generated, and given $x^n$ and $w^n$, we choose one of them if:
  \begin{equation}
  \left(u^n(m),w^n,x^n\right)\in\mathcal{T}^n_{[UWX]\epsilon},\ \mbox{for some}\ m\in[1:S] \ .\end{equation}
 If there are various vectors $u^n$ that satisfies this we choose the one with smallest index. If there are none we choose an arbitrary one. Let $M$ denote the index chosen. 
 %Assume that:
% \[\mbox{Pr}\left\{\left(U^n(m),W^n,X^n\right)\notin\mathcal{T}^n_{[UWX]\epsilon}\ \forall m\in[1:S]\right\}\xrightarrow[n\rightarrow\infty]{}0.\]
 Then we have that:
  \begin{equation}
 \mbox{Pr}\left\{U^n(M)=u^n\Big|x^n,w^n,U^n(M)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}=
 \frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|XW]\epsilon}^n(x^n,w^n)\right\}}{\|\mathcal{T}_{[U|XW]\epsilon}(x^n,w^n)\|} \ .
 \end{equation}
   \end{lemma}
   \begin{IEEEproof}
   From the selection procedure for $M$ we know that:
  \begin{equation}
  M=f\left(\mathds{1}\left\{(U^n(m),X^n,W^n)\in\mathcal{T}_{[UXW]\epsilon}^n\right\}, m\in[1:S]\right)\ , \end{equation}
   where $f(\cdot)$ is an appropriate function. Moreover, because of this and the way in which the random vectors $U^n$ are generated we have:
\begin{equation}
U^n(M)\mkv\left(\mathds{1}\left\{(U^n(M),X^n,W^n)\in\mathcal{T}_{[UXW]\epsilon}^n\right\},W^n,X^n\right)\mkv M\ .
\label{eq:mkv}
\end{equation}
We can write:
\begin{IEEEeqnarray}{lCl}
\mbox{Pr}\left\{U^n(M)=u^n\Big|x^n,w^n,U^n(M)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}=\nonumber\\
\sum_{m=1}^S\mbox{Pr}\left\{M=m\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}\times\nonumber\\
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n),M=m\right\}.
\label{eq:mkv2}
\end{IEEEeqnarray}
From (\ref{eq:mkv}), the second probability term in the RHS of (\ref{eq:mkv2}) can be written as:
\begin{equation}
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}\ \forall m\ .
\end{equation}
We are going to analyze this term. It is clear that we can write:
\begin{IEEEeqnarray}{rcl}
\mbox{Pr}\left\{U^n(m)=u^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\Big| x^n,w^n\right\} &=&
\mathds{1}\left\{u^n\in\mathcal{T}_{[U|WX]\epsilon}^n(x^n,w^n)\right\}\nonumber\\
& &\times\mbox{Pr}\left\{U^n(m)=u^n\Big| x^n,w^n\right\}\ \forall m\ .\,\,\, \,\, \, \,\, 
\end{IEEEeqnarray}
\end{IEEEproof}
This means that
\begin{gather}
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}\nonumber\\
=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|WX]\epsilon}^n(x^n,w^n)\cap\mathcal{T}_{[U|W]\epsilon'}^n(w^n)\right\}}{
\mbox{Pr}\left\{U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\Big| x^n,w^n\right\}\|\mathcal{T}_{[U|W]\epsilon'}(w^n)\|}\ \forall m
\label{eq:uniform_1}
\end{gather}
From (\ref{eq:uniform_1}) and the fact that for $\epsilon'\geq\epsilon$, we have that $\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\subseteq
\mathcal{T}^n_{[U|W]\epsilon'}(w^n)$ we obtain:
\begin{equation}
\mbox{Pr}\left\{U^n(m)=u^n\Big|x^n,w^n,U^n(m)\in\mathcal{T}^n_{[U|XW]\epsilon}(x^n,w^n)\right\}
=\frac{\mathds{1}\left\{u^n\in\mathcal{T}_{[U|WX]\epsilon}^n(x^n,w^n)\right\}}
{\|\mathcal{T}_{[U|XW]\epsilon}(x^n,w^n)\|}\ \forall m\ .
\label{eq:uniform_2}
\end{equation}
From this equation and (\ref{eq:mkv2}) we easily obtain the desired result.

%------------------------------------------------------------------------------
%\subsection{Csisz\'ar and K\"orner's Equality}
%
%
%\begin{lemma}[{Csisz\'ar and K\"orner's equality~\cite[Lemma~7]\cite{csiszar1978broadcast}}]\label{sec:csiszarkorner}
%Consider two  sequences $X^n$ and $Y^n$, and a random variable $Z$ arbitrarly distributed.
%The following identity holds true:
%\[
%\sum_{i=1}^n I(Y_{i+1}^n ; X_i | Z X^{i-1})
%	=	\sum_{j=1}^n I(X^{j-1} ; Y_j | Z Y_{j+1}^n)	\ .
%\]
%\end{lemma}

We present, without proof, a useful result about reconstruction functions for lossy source coding problems:
\begin{lemma}[Reconstruction functions for degraded random variables \cite{kaspi_two-way_1985}]
\label{lemma:Markov_distortion}
Consider random variables $(X,Y,Z)$ such that $X\mkv Y\mkv Z$. Consider an arbitrary function $\hat{X}=f(Y,Z)$ and an arbitrary positive distortion function $d(\cdot,\cdot)$. Then $\exists\ g^{*}(Y)$ such that
\begin{equation}
E\left[d(X,g^{*}(Y))\right]\leq E[d(X,f(Y,Z))]\ .
\label{eq:best_dist_function}
\end{equation}
\end{lemma}


==> figures/GaussianEqualMarginals.tex <==
\pgfplotsset{compat=newest}
\pgfkeys{/pgfplots/.cd,master axis/.style={
    scale only axis,
    enlarge x limits=false,
    axis x line*=bottom,
    xticklabel shift=3pt,
    after end axis/.code={
      \pgfkeys{/pgf/fpu=true,/pgf/fpu/output format=fixed}
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmin}}
      \global\let\masterxmin=\pgfmathresult
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmax}}
      \global\let\masterxmax=\pgfmathresult
      \pgfkeys{/pgf/fpu=false}
    },
  },
  slave axis/.style={
    scale only axis,enlarge x limits=false,
    axis x line*=top,
    axis y line=none,
    xmin=\masterxmin,xmax=\masterxmax,
    ymin=0,ymax=0.25,
    scaled x ticks=false,
    xtick={0,0.0457,0.1368,0.2172,0.2858,0.3446,0.3953,0.4394,0.459},
    xticklabels={0.75,0.7,0.6,0.5,0.4,0.3,0.2,0.1,0},
    %  \pgfkeys{/pgf/fpu}%
    %  \pgfmathparse{1/\tick}%
    %  \pgfmathprintnumber{\pgfmathresult}%
    %},
    %  xticklabel style={/pgf/number format/.cd,fixed,precision=2},
    %  xmajorgrids=true, % to show the tick position
    %  every axis x grid/.style={red,dashed,very thick},
  }
}
  % calculation of the xtick position
  %\xdef\slavextick{}
  %\foreach[count=\n][evaluate=\i as \j using 1/\i]%
  % \i in {0.12,0.11,...,0.07} % xtick for the slave axis
  %  {\pgfmathparse{\n==1?"":","}\xdef\slavextick{\slavextick\pgfmathresult\j}
  %  }

\begin{tikzpicture}

\begin{axis}[master axis,
  ymin=0,ymax=0.25,
  xmin=0,xmax=0.459,
  enlarge x limits=false,
  xlabel={$E$},
  ylabel=$D_0$,
]
\addplot[black,line width = 1pt] coordinates{
( 0.008, 0.115)( 0.016, 0.118)( 0.025, 0.121)( 0.033, 0.125)( 0.042, 0.128)( 0.050, 0.131)( 0.059, 0.134)( 0.067, 0.137)( 0.076, 0.140)( 0.084, 0.143)( 0.093, 0.146)( 0.101, 0.149)( 0.109, 0.152)( 0.117, 0.155)( 0.125, 0.158)( 0.133, 0.160)( 0.141, 0.163)( 0.149, 0.166)( 0.156, 0.168)( 0.164, 0.171)( 0.171, 0.173)( 0.178, 0.176)( 0.186, 0.178)( 0.193, 0.181)( 0.200, 0.183)( 0.207, 0.185)( 0.213, 0.188)( 0.220, 0.190)( 0.227, 0.192)( 0.233, 0.194)( 0.240, 0.196)( 0.246, 0.199)( 0.252, 0.201)( 0.258, 0.203)( 0.264, 0.205)( 0.270, 0.207)( 0.276, 0.209)( 0.282, 0.211)( 0.287, 0.213)( 0.293, 0.215)( 0.298, 0.217)( 0.304, 0.218)( 0.309, 0.220)( 0.315, 0.222)( 0.320, 0.224)( 0.325, 0.226)( 0.330, 0.227)( 0.335, 0.229)
};

\addplot[blue,line width = 1pt] coordinates{
( 0.009, 0.031)( 0.018, 0.033)( 0.028, 0.034)( 0.037, 0.035)( 0.047, 0.036)( 0.057, 0.037)( 0.067, 0.038)( 0.077, 0.039)( 0.087, 0.041)( 0.097, 0.042)( 0.107, 0.043)( 0.117, 0.044)( 0.127, 0.045)( 0.137, 0.046)( 0.147, 0.047)( 0.157, 0.048)( 0.166, 0.049)( 0.176, 0.050)( 0.185, 0.051)( 0.195, 0.052)( 0.204, 0.053)( 0.213, 0.055)( 0.222, 0.056)( 0.231, 0.057)( 0.240, 0.058)( 0.249, 0.059)( 0.258, 0.060)( 0.266, 0.061)( 0.275, 0.062)( 0.283, 0.063)( 0.291, 0.064)( 0.300, 0.065)( 0.308, 0.066)( 0.316, 0.067)( 0.324, 0.068)( 0.331, 0.069)( 0.339, 0.070)( 0.347, 0.071)( 0.354, 0.072)( 0.362, 0.073)( 0.369, 0.074)( 0.377, 0.075)( 0.384, 0.075)( 0.391, 0.076)( 0.398, 0.077)( 0.405, 0.078)( 0.412, 0.079)( 0.419, 0.080)
};

\addplot[red,line width = 1pt] coordinates{
( 0.009, 0.008)( 0.019, 0.008)( 0.029, 0.009)( 0.039, 0.009)( 0.049, 0.009)( 0.059, 0.010)( 0.069, 0.010)( 0.080, 0.010)( 0.090, 0.011)( 0.101, 0.011)( 0.111, 0.011)( 0.122, 0.011)( 0.132, 0.012)( 0.142, 0.012)( 0.153, 0.012)( 0.163, 0.013)( 0.173, 0.013)( 0.183, 0.013)( 0.193, 0.014)( 0.203, 0.014)( 0.213, 0.014)( 0.222, 0.015)( 0.232, 0.015)( 0.242, 0.015)( 0.251, 0.015)( 0.260, 0.016)( 0.270, 0.016)( 0.279, 0.016)( 0.288, 0.017)( 0.297, 0.017)( 0.306, 0.017)( 0.314, 0.018)( 0.323, 0.018)( 0.332, 0.018)( 0.340, 0.018)( 0.349, 0.019)( 0.357, 0.019)( 0.365, 0.019)( 0.373, 0.020)( 0.381, 0.020)( 0.389, 0.020)( 0.397, 0.020)( 0.405, 0.021)( 0.413, 0.021)( 0.421, 0.021)( 0.428, 0.022)( 0.436, 0.022)( 0.443, 0.022)
};

\addplot[green,line width = 1pt] coordinates{
( 0.009, 0.001)( 0.019, 0.001)( 0.029, 0.001)( 0.039, 0.001)( 0.049, 0.001)( 0.060, 0.001)( 0.070, 0.001)( 0.081, 0.001)( 0.091, 0.001)( 0.102, 0.001)( 0.113, 0.001)( 0.123, 0.001)( 0.134, 0.001)( 0.144, 0.001)( 0.155, 0.001)( 0.165, 0.001)( 0.175, 0.001)( 0.185, 0.001)( 0.196, 0.001)( 0.206, 0.001)( 0.216, 0.001)( 0.225, 0.001)( 0.235, 0.001)( 0.245, 0.001)( 0.255, 0.001)( 0.264, 0.001)( 0.273, 0.001)( 0.283, 0.001)( 0.292, 0.001)( 0.301, 0.001)( 0.310, 0.001)( 0.319, 0.001)( 0.328, 0.001)( 0.337, 0.001)( 0.346, 0.001)( 0.354, 0.001)( 0.363, 0.001)( 0.371, 0.001)( 0.379, 0.001)( 0.388, 0.001)( 0.396, 0.001)( 0.404, 0.001)( 0.412, 0.001)( 0.420, 0.001)( 0.428, 0.001)( 0.436, 0.001)( 0.443, 0.001)( 0.451, 0.001)
};

\legend{ {$R=1$},{$R=2$},{$R=3$}, {$R=5$}}
\end{axis}

\begin{axis}[slave axis,xlabel=$D_1$]\end{axis}

\end{tikzpicture}

==> figures/GaussianSimulation3.tex <==
\pgfplotsset{compat=newest}
\pgfkeys{/pgfplots/.cd,master axis/.style={
    scale only axis,
    enlarge x limits=false,
    axis x line*=bottom,
    xticklabel shift=3pt,
    after end axis/.code={
      \pgfkeys{/pgf/fpu=true,/pgf/fpu/output format=fixed}
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmin}}
      \global\let\masterxmin=\pgfmathresult
      \pgfmathparse{\pgfkeysvalueof{/pgfplots/xmax}}
      \global\let\masterxmax=\pgfmathresult
      \pgfkeys{/pgf/fpu=false}
    },
  },
  slave axis/.style={
    scale only axis,enlarge x limits=false,
    axis x line*=top,
    axis y line=none,
    xmin=\masterxmin,xmax=\masterxmax,
    ymin=0,ymax=1,
    scaled x ticks=false,
    xtick={0,0.0338,0.0668,0.0976,0.1258,0.1515,0.1750,0.1963,0.2158,0.2336,0.2500},
    xticklabels={2,1.8,1.6,1.4,1.2,1,0.8,0.6,0.4,0.2,0},
    %  \pgfkeys{/pgf/fpu}%
    %  \pgfmathparse{1/\tick}%
    %  \pgfmathprintnumber{\pgfmathresult}%
    %},
    %  xticklabel style={/pgf/number format/.cd,fixed,precision=2},
    %  xmajorgrids=true, % to show the tick position
    %  every axis x grid/.style={red,dashed,very thick},
  }
}
  % calculation of the xtick position
  %\xdef\slavextick{}
  %\foreach[count=\n][evaluate=\i as \j using 1/\i]%
  % \i in {0.12,0.11,...,0.07} % xtick for the slave axis
  %  {\pgfmathparse{\n==1?"":","}\xdef\slavextick{\slavextick\pgfmathresult\j}
  %  }

\begin{tikzpicture}

\begin{axis}[master axis,
  ymin=0,ymax=0.9,
  xmin=0,xmax=0.25,
  enlarge x limits=false,
  xlabel={$E$},
  ylabel=$D_0$,
]
\addplot[black,line width = 1pt] coordinates{
( 0.003, 0.607)( 0.007, 0.614)( 0.010, 0.622)( 0.014, 0.628)( 0.017, 0.635)( 0.021, 0.642)( 0.024, 0.649)( 0.028, 0.655)( 0.031, 0.662)( 0.035, 0.668)( 0.038, 0.674)( 0.041, 0.680)( 0.045, 0.686)( 0.048, 0.692)( 0.052, 0.698)( 0.055, 0.704)( 0.058, 0.710)( 0.062, 0.715)( 0.065, 0.721)( 0.068, 0.726)( 0.071, 0.732)( 0.075, 0.737)( 0.078, 0.742)( 0.081, 0.747)( 0.084, 0.753)( 0.087, 0.758)( 0.090, 0.763)( 0.093, 0.767)( 0.096, 0.772)( 0.099, 0.777)( 0.102, 0.782)( 0.105, 0.786)( 0.108, 0.791)( 0.111, 0.796)( 0.114, 0.800)( 0.117, 0.804)( 0.120, 0.809)( 0.122, 0.813)( 0.125, 0.817)( 0.128, 0.822)( 0.131, 0.826)( 0.133, 0.830)( 0.136, 0.834)( 0.139, 0.838)( 0.141, 0.842)( 0.144, 0.846)( 0.146, 0.850)( 0.149, 0.853)
};

\addplot[blue,line width = 1pt] coordinates{
( 0.004, 0.180)( 0.009, 0.183)( 0.013, 0.186)( 0.018, 0.189)( 0.022, 0.192)( 0.027, 0.195)( 0.031, 0.198)( 0.036, 0.201)( 0.041, 0.204)( 0.045, 0.208)( 0.050, 0.211)( 0.055, 0.214)( 0.060, 0.217)( 0.064, 0.220)( 0.069, 0.222)( 0.074, 0.225)( 0.079, 0.228)( 0.083, 0.231)( 0.088, 0.234)( 0.093, 0.237)( 0.098, 0.240)( 0.102, 0.243)( 0.107, 0.246)( 0.112, 0.249)( 0.116, 0.251)( 0.121, 0.254)( 0.126, 0.257)( 0.130, 0.260)( 0.135, 0.263)( 0.139, 0.265)( 0.144, 0.268)( 0.149, 0.271)( 0.153, 0.274)( 0.158, 0.276)( 0.162, 0.279)( 0.166, 0.282)( 0.171, 0.284)( 0.175, 0.287)( 0.180, 0.290)( 0.184, 0.292)( 0.188, 0.295)( 0.193, 0.298)( 0.197, 0.300)( 0.201, 0.303)( 0.205, 0.306)( 0.209, 0.308)( 0.214, 0.311)( 0.218, 0.313)
};

\addplot[red,line width = 1pt] coordinates{
( 0.004, 0.047)( 0.009, 0.048)( 0.014, 0.049)( 0.019, 0.050)( 0.023, 0.051)( 0.028, 0.052)( 0.033, 0.053)( 0.038, 0.053)( 0.043, 0.054)( 0.048, 0.055)( 0.053, 0.056)( 0.058, 0.057)( 0.064, 0.058)( 0.069, 0.059)( 0.074, 0.060)( 0.079, 0.061)( 0.084, 0.062)( 0.089, 0.062)( 0.094, 0.063)( 0.100, 0.064)( 0.105, 0.065)( 0.110, 0.066)( 0.115, 0.067)( 0.120, 0.068)( 0.125, 0.069)( 0.130, 0.070)( 0.136, 0.070)( 0.141, 0.071)( 0.146, 0.072)( 0.151, 0.073)( 0.156, 0.074)( 0.161, 0.075)( 0.166, 0.076)( 0.171, 0.077)( 0.176, 0.077)( 0.181, 0.078)( 0.186, 0.079)( 0.190, 0.080)( 0.195, 0.081)( 0.200, 0.082)( 0.205, 0.083)( 0.210, 0.084)( 0.215, 0.084)( 0.219, 0.085)( 0.224, 0.086)( 0.229, 0.087)( 0.233, 0.088)( 0.238, 0.089)
};

\addplot[green,line width = 1pt] coordinates{
( 0.005, 0.003)( 0.009, 0.003)( 0.014, 0.003)( 0.019, 0.003)( 0.024, 0.003)( 0.029, 0.003)( 0.034, 0.003)( 0.039, 0.003)( 0.044, 0.003)( 0.049, 0.004)( 0.054, 0.004)( 0.060, 0.004)( 0.065, 0.004)( 0.070, 0.004)( 0.075, 0.004)( 0.081, 0.004)( 0.086, 0.004)( 0.091, 0.004)( 0.097, 0.004)( 0.102, 0.004)( 0.107, 0.004)( 0.112, 0.004)( 0.118, 0.004)( 0.123, 0.004)( 0.128, 0.004)( 0.134, 0.004)( 0.139, 0.005)( 0.144, 0.005)( 0.149, 0.005)( 0.154, 0.005)( 0.160, 0.005)( 0.165, 0.005)( 0.170, 0.005)( 0.175, 0.005)( 0.180, 0.005)( 0.185, 0.005)( 0.190, 0.005)( 0.195, 0.005)( 0.200, 0.005)( 0.205, 0.005)( 0.210, 0.005)( 0.215, 0.005)( 0.220, 0.005)( 0.225, 0.006)( 0.230, 0.006)( 0.235, 0.006)( 0.240, 0.006)( 0.245, 0.006)
};

\legend{ {$R=1$},{$R=2$},{$R=3$}, {$R=5$}}
\end{axis}

\begin{axis}[slave axis,xlabel=$D_1$]\end{axis}

\end{tikzpicture}

==> packages-2.tex <==

%--------------------------------------------------------------------
% packages standards
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{times}
\usepackage{graphicx}
\usepackage{color}
\usepackage{verbatim}
\usepackage{cite}

%--------------------------------------------------------------------
% autres packages

% pour les figures
\usepackage{subfig}		
%\usepackage{pgf}		
%\usepackage{tikz}
%\usepackage{pgfplots}	
%\usetikzlibrary{decorations}
%\usetikzlibrary{patterns}
%\usetikzlibrary{positioning}
%\usetikzlibrary{backgrounds}
%\usetikzlibrary{fit}
%\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{shapes.symbols}
%\usetikzlibrary{calc}

%--------------------------------------------------------------------
% pour passer temporairement en paysage
% \usepackage{pdflscape}
% \usepackage{lscape}

%--------------------------------------------------------------------
% pour \minuso
\usepackage{stmaryrd}

%--------------------------------------------------------------------
% pour barrer ie, simplifier des termes
\usepackage{cancel}
\usepackage[normalem]{ulem}

%--------------------------------------------------------------------
% pour commenter des blocs
\usepackage{verbatim}

%--------------------------------------------------------------------
\newtheorem{definition}	{Definition}
\newtheorem{theorem}	{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}		{Lemma}
\newtheorem{corollary}	{Corollary}
\newtheorem{remark}		{Remark}


==> packages.tex <==

%--------------------------------------------------------------------
% packages standards
\usepackage[latin1]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{times}
\usepackage{graphicx}
\usepackage{color}
\usepackage{verbatim}
\usepackage{cite}

%--------------------------------------------------------------------
% autres packages

% pour les figures
\usepackage{subfig}		
%\usepackage{pgf}		
%\usepackage{tikz}
%\usepackage{pgfplots}	
%\usetikzlibrary{decorations}
%\usetikzlibrary{patterns}
%\usetikzlibrary{positioning}
%\usetikzlibrary{backgrounds}
%\usetikzlibrary{fit}
%\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{shapes.symbols}
%\usetikzlibrary{calc}

%--------------------------------------------------------------------
% pour passer temporairement en paysage
% \usepackage{pdflscape}
% \usepackage{lscape}

%--------------------------------------------------------------------
% pour \minuso
\usepackage{stmaryrd}

%--------------------------------------------------------------------
% pour barrer ie, simplifier des termes
\usepackage{cancel}
\usepackage[normalem]{ulem}

%--------------------------------------------------------------------
% pour commenter des blocs
\usepackage{verbatim}

%--------------------------------------------------------------------
\newtheorem{definition}	{Definition}
\newtheorem{theorem}	{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}		{Lemma}
\newtheorem{corollary}	{Corollary}
\newtheorem{remark}		{Remark}

